Multi-Tubal Rank of Third Order Tensor and Related Low Rank Tensor Completion Problem

Recently, a tensor factorization based method for a low tubal rank tensor completion problem of a third order tensor was proposed, which performed better than some existing methods. Tubal rank is only defined on one mode of third order tensor without low rank structure in the other two modes. That is, low rank structures on the other two modes are missing. Motivated by this, we first introduce multi-tubal rank, and then establish a relationship between multi-tubal rank and Tucker rank. Based on the multi-tubal rank, we propose a novel low rank tensor completion model. For this model, a tensor factorization based method is applied and the corresponding convergence anlysis is established. In addition, spatio-temporal characteristics are intrinsic features in video and internet traffic tensor data. To get better performance, we make full use of such features and improve the established tensor completion model. Then we apply tensor factorization based method for the improved model. Finally, numerical results are reported on the completion of image, video and internet traffic data to show the efficiency of our proposed methods. From the reported numerical results, we can assert that our methods outperform the existing methods.

==> Chapter/section1.tex <==
\section{Introduction}
A tensor is a multidimensional array. More precisely, an N-way is an element of the tensor product of N vector spaces, each of which has its own coordinate system\cite{ref35}. Recently, a variety of high-dimensional data has appeared in the fields of physics, chemistry, and information science. The emergence of these high-dimensional data has led to an increasing understanding of high-dimensional data. The more complex the data we face, the larger the scale we need to process. Tensors, as high-level generalizations of vectors and matrices, can well characterize the high-dimensional complex data generated in the above fields. Research on Tensors and Their Applications Is Paying More and More Attention\cite{ref35}. However, in daily life, people often only obtain partial data when observing or collecting. In order to fill in the missing terms of some observed low-rank tensors, a low-rank tensor completion model has been proposed. Its mathematical model is written as
\begin{equation}\label{gs1.1}
\mathop {\min }\limits_{\mathcal C} \operatorname{rank} (\mathcal C),\quad s.t. \, {P_\Omega }({\mathcal C}) = {P_\Omega }(\mathcal M).
\end{equation}

where the set of positions $ \Omega $ corresponds to the observed data. $ P_\Omega $ is a linear operator that extracts the entries in $ \Omega $ and sets the data not in $ \Omega $ to zeros. The rank$ (\cdot) $ is the tensor rank function. However, the rank of tensor has different definition methods, and different definition methods correspond to different recovery algorithms. For instance, the CANDECOMP/PARAFAC(CP) rank \cite{ref30} of a tensor ${\mathcal{C}} \in {\mathbb{R}^{{n_1} \times {n_2} \times  \cdots {n_N}}}$ which is defined as the smallest number of rank one decomposition, i.e.
$$ran{k_{CP}}(\mathcal{C}) = \min \left\{ {\left. r \right|\mathcal{C} = \sum\limits_{i = 1}^r {a_1^{(i)} \otimes a_2^{(i)} \cdots  \otimes a_k^{(i)}} } \right\}.$$
where the symbol $ \otimes $ denotes the outer product and $a_j^{(i)}$ is a vector. Unfortunately, this tensor rank is difficult to handle, because there is no direct algorithm to determine the $ ran{k_{CP}} $ of a given tensor. In fact, this problem is generally NP-hard to compute\cite{ref16}. Another concept is Tucker rank, which is easy to calculate. Its formula is defined as
$$ran{k_{TC}}(\mathcal{C}) = \left( {rank({\mathcal{C}_{(1)}}),rank({\mathcal{C}_{(2)}}), \cdots ,rank({\mathcal{C}_{(N)}})} \right).$$
where $ \mathcal{C}_{(i)} $ is its mode-$ i $ matricization. Based on Tucker rank, S. Gandy and others consider the following minimization problems \cite{ref314}
\begin{equation}\label{gs1.2}
\mathop {\min }\limits_{\mathcal{C}} \sum\limits_{i = 1}^k rank({{\mathcal{C}_{(i)}}})  ,\quad s.t. \, {P_\Omega }({\mathcal C}) = {P_\Omega }(\mathcal M).
\end{equation}
The rank minimization problem \eqref{gs1.2} is a difficult non-convex problem due to the combined nature of the function rank $ (\cdot) $. Therefore, we will replace the rank $ (\cdot) $ with its convex nuclear norm, and obtain a convex and easier to compute approximation to \eqref{gs1.2} yields the low Tucker rank
tensor pursuit problem
\begin{equation}\label{gs1.3}
\mathop {\min }\limits_{\mathcal{C}} \sum\limits_{i = 1}^k {{{\left\| {{{\mathcal C}_{(i)}}} \right\|}_*}} ,\quad s.t. \, {P_\Omega }({\mathcal C}) = {P_\Omega }(\mathcal M).
\end{equation}
However, the nuclear norm minimization problem \eqref{gs1.3} is generally an iterative solution, and each iteration involves SVD. Therefore, these nuclear norm minimization methods face high computational costs for multiple SVDs. In order to efficiently process large-scale data, Xu et al. \cite{ref3} used a matrix decomposition method to preserve the low rank structure of the unexpanded matrix, that is, decompose each pattern matrix $ {C} _{(i)} $ into the product of two smaller matrices $ X^{i} $ and $ Y^{i} $:
\begin{equation}\label{gs1.4}
\mathop {\min }\limits_{{X^i},{Y^i},{\mathcal C}} \sum\limits_{i = 1}^k {{\alpha _i}{{\left\| {{X^i}{Y^i} - {{\mathcal C}_{(i)}}} \right\|}_*}} ,\quad s.t. \, {P_\Omega }({\mathcal C}) = {P_\Omega }(\mathcal M).
\end{equation}
This method has been widely used in various applications \cite{ref10}. However, directly expanding a tensor will destroy the original internal structure of the data, leading to the loss of internal cross-information. In addition, each module-i matrix has the same number of terms as the tensor, and then each module-i matrix is restored and merged into a tensor in each iteration, which may be inefficient because  the number of tensor items is usually large. Recently, Kilmer et al.\cite{ref33} defined tensor-tensor product and tensor singular value decomposition based on tensor-tensor product and tensor singular value decomposition \cite{ref36,ref37,ref38}. Semerci et al.\cite{ref34} proposed a new tensor nuclear norm (TNN). Subsequently, Zhang et al. applied TNN to tensor completion \cite{ref1},  Since $ T $-SVD is based on an operator theoretic interpretation of 3-way tensors as linear operators on the space of oriented matrices, Tensor multi-rank and tubal rank  very effectively describe the inherent low-rank structure of the tensor, while avoiding the shortcomings of the internal relationships of the data lost by tensor matrixization \cite{ref33,ref36,ref37}. But TNN still needs to calculate $ T $-SVD, which is very time consuming when the data size is large. Therefore, Zhou et al. \cite{ref} decomposes the low-rank tensor ${\mathcal{C}} \in {\mathbb{R}^{{n_1} \times {n_2} \times {n_3}}}$ into the product of two smaller tensors ${\mathcal X} \in {{\mathbb{R}}^{{n_1} \times r \times {n_3}}}$ and ${\mathcal Y} \in {\mathbb{R}^{r \times {n_2} \times {n_3}}}$. 
\begin{equation}\label{gs1.5}
\mathop {\min }\limits_{\mathcal{X},\mathcal{Y},\mathcal{C}} \frac{1}{2}\left\| {\mathcal{X}*\mathcal{Y} - \mathcal{C}} \right\|_F^2,\quad s.t. \, {P_\Omega }(\mathcal{C} - \mathcal{M}) = 0.
\end{equation}
This low-rank decomposition method(TCTF) avoids calculating $ T $-SVD, which is very efficient. However, the tensor tubal rank only considers the
frontal slice of the tensor, and ignores the role of horizontal slice and lateral slice, So the more missing tensor data, the worse the recovery effect.
\par In this paper, we proposes a new generalized tubal rank method to solve the 3-way tensor completion problem. Similar to TCTF \cite{ref}, our method is also based on the tensor multi-rank and tubal rank definitions. We also decompose the low-rank tensor ${\mathcal{C}} \in {\mathbb{R}^{{n_1} \times {n_2} \times {n_3}}}$ into the product of two smaller tensors ${\mathcal X} \in {{\mathbb{R}}^{{n_1} \times r \times {n_3}}}$ and ${\mathcal Y} \in {\mathbb{R}^{r \times {n_2} \times {n_3}}}$. However, we define the tensor multi-rank matrix and tubal rank vector, and also consider the information of the horizontal, lateral and frontal slices of the tensor $ {\mathcal{C}} $, so we can more fully characterize the low rank property of the tensor $ {\mathcal{C}} $ and restore it. Because we describe the tensor multi-rank matrix and tubal rank vector, the structure of the tensor is more comprehensively considered, which is much better than the result of TCTF. Compared with the method based on tensor turck rank, our method is based on the tensor multi-rank matrix and tubal rank vector, which avoids the loss of low-rank structure information. The experimental results also confirm this. We also propose a regularization method that avoids the generalized inverse of the calculation matrix and makes the calculation more efficient. \textcolor{red}{In addition, we have also improved the algorithm for data with certain spatiotemporal characteristics.} 
Finally, we propose an efficient optimization method for solving our model, and further prove its convergence.

==> Chapter/section2.tex <==
\section{Preliminaries}
\setcounter{equation}{0}
In this section, we first briefly summarize some main notations and then introduce some definitions and a lemma used later in this paper.
\subsection{Notations}
\textcolor{red}{ add $ \to $Throughout the paper, we let $ [n] = {1,2,\cdots, n} $.  } We use lowercase letters, e.g. $  a,b,c,\cdots, $ to denote scalars, and boldface lowercase letters, e.g. $\bm{a} ,\bm{b},\bm{c},\cdots, $ to represent vectors. And matrices by uppercase letters, e.g. $ A,B,C,\cdots $, A 3-way tensor is denoted as $ \mathcal{A},\mathcal{B},\mathcal{C},\cdots $. For a 3-way tensor $ \mathcal{A} $, we use the Matlab notation $ \mathcal{A}(i,:, :), \mathcal{A}(:, j, :) $ and $  \mathcal{A}(:, :, k)  $ to denote its $ i $-th horizontal, lateral and frontal slice, respectively. Let $\A=(\A_{ijk})\in \R^{n_1\times n_2\times n_3},$ $(A_1^{(i)})_{jk} = (A_2^{(j)})_{ik}=(A_3^{(k)})_{ij}=\A_{ijk}$ for all $i\in [n_1]$, $j\in [n_2]$ and $k\in [n_3]$. The inner product of two 3-way tensors  $ \mathcal{A},\mathcal{B} \in {R^{{n_1} \times {n_2} \times {n_3}}}$ is the sum of the products of their entries, i.e.
$$\left\langle {\mathcal{A},\mathcal{B}} \right\rangle  = \sum\limits_{i = 1}^{{n_1}} {\sum\limits_{j = 1}^{{n_2}} {\sum\limits_{k = 1}^{{n_3}} {{\mathcal{A}_{ijk}}{\mathcal{B}_{ijk}}} } }. $$
The corresponding (Frobenius-) norm is ${\left\| \mathcal{A} \right\|_F} = \sqrt {\left\langle {\mathcal{A},\mathcal{A}} \right\rangle } $. $ {\left\| \mathcal{A} \right\|_{\infty}} $   represents the maximum absolute value in $\mathcal{A}  $. $ A^* $ and $ A^\dagger $ represent the conjugate transpose and the pseudo-inverse of $ A $, respectively. $ I_n $ represents the identity matrix of size $ n \times n $.




\iffalse

\par Next, we introduce the Discrete Fourier Transformation
(DFT), which plays a core role in tensor-tensor product
introduced later. Let ${{\bar {\mathcal A}}_u} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$ represent the result of
Discrete Fourier transformation (DFT) of ${{ {\mathcal A}}} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$
along the $ u $-th dimension. Define the DFT matrix groups: $F, G, H $ are matrices of dimension $n_1, n_2$ and $n_3$, respectively.  
Here, DFT matrix have the following form
\begin{equation*}
\begin{aligned}
F_{n_u}\left[ {{f_1}, \cdots ,{f_i}, \cdots ,{f_{{n_u}}}} \right] \in {\mathbb R}^{{n_u} \times {n_u}}.
\end{aligned}
\end{equation*}
\iffalse
\begin{equation*}
\begin{aligned}
 F_{{n_1}} &= \left[ {{f_1}, \cdots ,{f_i}, \cdots ,{f_{{n_1}}}} \right] \in {\mathbb R}^{{n_1} \times {n_1}}, \\
 G_{{n_2}} &= \left[ {{g_1}, \cdots ,{g_i}, \cdots ,{g_{{n_2}}}} \right] \in {\mathbb R}^{{n_2} \times {n_2}},  \\
H_{{n_3}} &= \left[ {{h_1}, \cdots ,{h_i}, \cdots ,{h_{{n_3}}}} \right] \in {\mathbb R}^{{n_3} \times {n_3}}. 
\end{aligned}
\end{equation*}

where
\begin{equation*}
\begin{aligned}
{f_i} &= \left[ {{\omega_1 ^{0 \times (i - 1)}};{\omega_1 ^{1 \times (i - 1)}}; \cdots ;{\omega_1 ^{\left( {{n_1} - 1} \right) \times (i - 1)}}} \right] \in {{\mathbb R}^{{n_1}}},  \\
 {g_i} &= \left[ {{\omega_2 ^{0 \times (i - 1)}};{\omega_2 ^{1 \times (i - 1)}}; \cdots ;{\omega_2 ^{\left( {{n_2} - 1} \right) \times (i - 1)}}} \right] \in {{\mathbb R}^{{n_2}}},\\
 {h_i} &= \left[ {{\omega_3 ^{0 \times (i - 1)}};{\omega_3 ^{1 \times (i - 1)}}; \cdots ;{\omega_3 ^{\left( {{n_3} - 1} \right) \times (i - 1)}}} \right] \in {{\mathbb R}^{{n_3}}}. 
\end{aligned}
\end{equation*}
\fi

where
\begin{equation*}
\begin{aligned}
{f_i} &= \left[ {{\omega_u ^{0 \times (i - 1)}};{\omega_u ^{1 \times (i - 1)}}; \cdots ;{\omega_u ^{\left( {{n_u} - 1} \right) \times (i - 1)}}} \right] \in {{\mathbb R}^{{n_u}}}
\end{aligned}
\end{equation*}


in which ${\omega_u} = {e^{ - (2\pi b/{n_u})}},u \in [3].$ and $b = \sqrt { - 1} $.
\par Clearly,
\[ {{\bar {\mathcal A}}_1}=F_{n_{1}}\times_1{\mathcal A}, \quad {{\bar {\mathcal A}}_2}=G_{n_{2}}\times_2{\mathcal A},\quad {{\bar {\mathcal A}}_3}=H_{n_{3}}\times_3{\mathcal A}. \]





\[ {{\bar {\mathcal A}}_1}=F_{n_{1}}{\mathcal A}(:,j,k),{{\bar {\mathcal A}}_2}=G_{n_{2}}{\mathcal A}(i,:,k),{{\bar {\mathcal A}}_3}=H_{n_{3}}{\mathcal A}(i,j,:). \]


\fi



\par Next, we introduce the Discrete Fourier Transformation
(DFT), which plays a core role in tensor-tensor product
introduced later. Let ${{\bar {\mathcal A}}_u} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$ represent the result of
Discrete Fourier transformation (DFT) of ${{ {\mathcal A}}} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$
along the $ u $-th dimension. Indeed, we can compute $ {{\bar {\mathcal A}}_u} $ directly by the Matlab command $ {{\bar {\mathcal A}}_u}=fft({\mathcal A},[],u)$ and use the inverse DFT to obtain $ {\mathcal A}=ifft({\bar {\mathcal A}}_u,[],u) $. We further define separately ${{\bar A}_1} \in {{\mathbb C}^{{n_1}{n_2} \times {n_1}{n_3}}},{{\bar A}_2} \in {{\mathbb C}^{{n_1}{n_2} \times {n_2}{n_3}}},{{\bar A}_3} \in {{\mathbb C}^{{n_1}{n_3} \times {n_2}{n_3}}}$ as 
\[{{\bar A}_u} = bdiag_{u}({{\bar {\mathcal A}}}) = \left[ {\begin{array}{*{20}{c}}
	{\bar A_u^1}&{}&{}&{}\\
	{}&{\bar A_u^2}&{}&{}\\
	{}&{}& \ddots &{}\\
	{}&{}&{}&{\bar A_u^{{n_u}}}
	\end{array}} \right],u \in [3].\]
where  $ bdiag_{u}(\cdot) $ is an operator which maps the tensor $ {{\bar {\mathcal A}}} $ to the block diagonal matrix $ {{\bar A}_u} $. We further define separately the block circulant matrix $bcirc_{1}({{\mathcal A}}) \in {{\mathbb C}^{{n_1}{n_2} \times {n_1}{n_3}}},bcirc_{2}({{\mathcal A}}) \in {{\mathbb C}^{{n_1}{n_2} \times {n_2}{n_3}}},bcirc_{3}({{\mathcal A}}) \in {{\mathbb C}^{{n_1}{n_3} \times {n_2}{n_3}}}$ of $ {{\bar {\mathcal A}}} $ as
\[bcirc_{u}({{\mathcal A}}) = \left[ {\begin{array}{*{20}{c}}
	{A_u^{(1)}}&{A_u^{({n_u})}}& \cdots &{A_u^{(2)}}\\
	{A_u^{(2)}}&{A_u^{(1)}}& \cdots &{A_u^{(3)}}\\
	\vdots & \vdots & \ddots & \vdots \\
	{A_u^{({n_u})}}&{A_u^{({n_u} - 1)}}& \cdots &{A_u^{(1)}}
	\end{array}} \right],u \in [3].\]
\iffalse
The definitions of $ {{\bar A}_u} $ and $ bcirc_{u}({{\mathcal A}}) $ are the basis of tensor rank and nuclear norm that will be introduced subsequently.
\fi

\subsection{Basic Knowledge}
We first introduce $ T_u $-product between two 3-way tensors.

\iffalse
\begin{definition}\label{definition2.1}
\textbf{(General $ \bm{T} $-produc)} The $ T_j $-product $ (j=1,2,3) $ between $ {\mathcal A_j} $ and $ {\mathcal B_j} $ is defined as ${\mathcal A_j}{ \times _j}{\mathcal B_j} = fold(bcirc({{\mathcal A}_j}) \cdot unfold({{\mathcal B}_j}))$, where 
\[ unfold_{j}({{\mathcal B}}) = [B_j^{(1)};B_j^{(2)}; \cdots ;B_j^{({n_j})}]. \] 
and its inverse operator fold$ _{j} $ is defined as $fold_{j}(unfold_{j}({{\mathcal B}})) = {{\mathcal B}}$. When $ j = 3 $, it degenerates to the \textbf{ $ \bm{T} $-produc}\cite{KM11}.
\end{definition}
Indeed, $ T_j $-product is equivalent to the matrix multiplication
in the Fourier domain, $ i.e. $ ${\mathcal F_j} = {\mathcal A_j}{ \times _j}{\mathcal B_j}$ and ${{\bar F}_j} = {{\bar A}_j}{{\bar B}_j}$ are
equivalent. When $ j = 3 $, it degenerates to the T-product\cite{KM11}, ( see Lemma 1). Based on the definition of $ T_j $-product, we introduce the definition of $ T_j $-SVD. Before that, we also need some other concepts.

\begin{definition}\label{definition2.2}
\textbf{(General $ \bm{F} $-diagonal tensor)}  A tensor is called $ f_1 (f_2,f_3) $-diagonal if each of its horizontal(lateral , frontal) slices is a diagonal matrix. When $ j = 3 $, it degenerates to the \textbf{$ \bm{F} $-diagonal tensor}\cite{KM11}.
\end{definition}

\begin{definition}\label{definition2.3}{\bfseries (General Conjugate transpose) }  The conjugate transpose of a tensor ${\mathcal A} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$ is the tensor${{\mathcal A}^{{*_1}}} \in {{\mathbb C}^{{n_1} \times {n_3} \times {n_2}}}({{\mathcal A}^{{*_2}}} \in {{\mathbb C}^{{n_3} \times {n_2} \times {n_1}}},{{\mathcal A}^{{*_3}}} \in {{\mathbb C}^{{n_2} \times {n_1} \times {n_3}}})$ obtained by conjugate transposing each of the
horizontal(lateral , frontal) slices and then reversing the order of transposed horizontal(lateral , frontal) slices $ 2 $ through $ n_{1}(n_{2},n_{3}) $. When $ j = 3 $, it degenerates to the {\bfseries Conjugate transpose}\cite{KM11}.
\end{definition}

\begin{definition}\label{definition2.4}{\bfseries (General Identity tensor) } The identity tensor ${\mathcal I^1} \in {{\mathbb C}^{{n_1} \times n \times n}}$ $({\mathcal I^2} \in {{\mathbb C}^{n \times {n_2} \times n}},{\mathcal I^3} \in {{\mathbb C}^{n \times n \times {n_3}}})$ is the tensor whose first horizontal(lateral , frontal) slice is the $ n \times n $ identity matrix, and other horizontal(lateral , frontal) slices are all zeros. When $ j = 3 $, it degenerates to the {\bfseries Identity tensor}\cite{KM11}.
\end{definition}

\begin{definition}\label{definition2.5}{\bfseries (General Orthogonal tensor) }  A tensor ${\mathcal P_1} \in {{\mathbb C}^{{n_1} \times n \times n}}$ $({\mathcal P_2} \in {{\mathbb C}^{n \times {n_2} \times n}}, {\mathcal P_3} \in {{\mathbb C}^{n \times n \times {n_3}}})$ is orthogonal if it satisfies 
	\[ {\mathcal P}_j^{{*_j}}{ \times _j}{\mathcal P_j} = {\mathcal P_j}{ \times _j}{\mathcal P}_j^{{*_j}} = {\mathcal I^j}. \, (j = 1,2,3) \]	
\end{definition}
When $ j = 3 $, it degenerates to the {\bfseries Orthogonal tensor}\cite{KM11}.
Now we introduce the recently proposed General $ T_j $-SVD, a new tensor decomposition framework.

\begin{theorem}\label{theorem2.1}{\bfseries (General $ T $-SVD) } Assume that ${\mathcal A} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$ is a 3-way tensor. Then it can be factored as 
\begin{equation}\label{gs2.1}
{\mathcal A} = {{\mathcal U}_j}{ \times _j}{{\mathcal S}_j}{ \times _j}{{\mathcal V}_j^{{*_j}}}. \, (j = 1,2,3)
\end{equation}
where ${{\mathcal U}_1} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_2}}}({{\mathcal U}_2} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_1}}},{{\mathcal U}_3} \in {{\mathbb C}^{{n_1} \times {n_1} \times {n_3}}})$ and ${{\mathcal V}_1} \in {{\mathbb C}^{{n_1} \times {n_3} \times {n_3}}}({{\mathcal V}_2} \in {{\mathbb C}^{{n_3} \times {n_2} \times {n_3}}},{{\mathcal V}_3} \in {{\mathbb C}^{{n_2} \times {n_2} \times {n_3}}})$ are orthogonal tensors, and ${{\mathcal S}_j}(j = 1,2,3) \in {{\mathbb C}^{{n_1} \times {n_{\text{2}}} \times {n_3}}}$ is a $ f_j $-diagonal tensor. When $ j = 3 $, it degenerates to the {\bfseries $ T $-SVD}\cite{KM11}.
\end{theorem}

$ T_j $-SVD employs similar properties to matrix SVD, such as
the orthogonal property of $ U_j $ and $ V_j $, and the diagonal structure of $ S_j $. Indeed, when $ n_{j} = 1 $, $ T_j $-SVD would degrade into matrix SVD. Now we introduce tensor multi-rank matrix and tubal rank vector.

\begin{definition}\label{definition2.6}{\bfseries (tensor multi-rank matrix and tubal rank vector) } For any ${\mathcal A} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$, its multi-rank matrix $rank_m({\mathcal A})$ is a matrix defined as $R=ran{k_m}({\mathcal A}) = (rank_m^1({\mathcal A}),rank_m^2({\mathcal A}),rank_m^3({\mathcal A}))$, where
$$rank_m^j({\mathcal A}) = \bm{r^j} = \left( {rank\left( {\bar A_j^{(1)}} \right),rank\left( {\bar A_j^{(2)}} \right), \cdots ,rank\left( {\bar A_j^{({n_j})}} \right)} \right). \, (j=1,2,3)$$
The tensor tubal rank  vector $ran{k_t}({\mathcal A})$ is a vector defined as 
\[ ran{k_t}({\mathcal A}) = (rank_t^1({\mathcal A}),rank_t^2({\mathcal A}),rank_t^3({\mathcal A})). \]
 where $ran{k_t^j}({\mathcal A})$ is defined as the number of nonzero singular tubes of $ {\mathcal S}_j $, i.e.
\begin{equation*}
\begin{aligned}
rank_t^1({\mathcal A}) &= \# \left\{ {i:{S_1}(:,i,i) \ne 0} \right\} = \max (\bm{r_1^1},\bm{r_2^1}, \cdots ,\bm{r_{{n_1}}^1}),\\
rank_t^2({\mathcal A}) &= \# \left\{ {i:{S_1}(i,:,i) \ne 0} \right\} = \max (\bm{r_1^2},\bm{r_2^2}, \cdots ,\bm{r_{{n_2}}^2}),\\
rank_t^3({\mathcal A}) &= \# \left\{ {i:{S_1}(i,i,:) \ne 0} \right\} = \max (\bm{r_1^3},\bm{r_2^3}, \cdots ,\bm{r_{{n_3}}^3}).
\end{aligned}
\end{equation*}	
When $ j = 3 $, it degenerates to the {\bfseries tensor multi-rank and tubal rank }\cite{KBHH13}.
\end{definition}
Then we can give the definition of tensor nuclear norm,
which is the convex envelop of the tensor average rank. With
this property, we use tensor nuclear norm to depict the lowrank structure of a tensor.

\begin{definition}\label{definition2.7}{\bfseries (Tensor nuclear norm) }  The tensor nuclear norm ${\left\| {\mathcal A} \right\|_*}$ of a tensor ${\mathcal A} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$ is defined as
$${\left\| {\mathcal A} \right\|_*} = \sum\limits_{j = 1}^3 {\frac{{{\alpha _j}}}{{{n_j}}}\sum\limits_{i = 1}^{{n_j}} {{{\left\| {\bar A_j^{(i)}} \right\|}_*}} }  = \sum\limits_{j = 1}^3 {\sum\limits_{i = 1}^{{n_j}} {\frac{{{\alpha _j}}}{{{n_j}}}{{\left\| {\bar A_j^{(i)}} \right\|}_*}} }. $$	
\end{definition}

Finally, we introduce a lemma which will be used for model
simplification and theoretical analysis.

\fi

\begin{definition}\label{def:T-pro}
	\textbf{(Generalized $\bm{T}_u$-product)} The generalized $T_u$-product $ (u \in [3]) $ between $ {\mathcal A_u} $ and $ {\mathcal B_u} $ is defined as ${\mathcal A_u}{ \times _u}{\mathcal B_u} = fold(bcirc({{\mathcal A}_u}) \cdot unfold({{\mathcal B}_u}))$, where
	\[ unfold_{u}({{\mathcal B}}) = [B_u^{(1)};B_u^{(2)}; \cdots ;B_u^{({n_u})}]. \]
	and its inverse operator fold$ _{u} $ is defined as $fold_{u}(unfold_{u}({{\mathcal B}})) = {{\mathcal B}}$.
\end{definition}

Now we introduce Multi-tubal rank vector.

\begin{definition}\label{definition2.6}{\bfseries (Multi-tubal rank vector)} For any ${\mathcal A} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$, let $r_u^l=r(\bar A_u^{(l)})$ for all $u\in [3]$ and $l\in [n_u]$.
	Then multi-tubal rank of $\A$ is defined as \[rank_{mt}(\A)=(r_1,r_2,r_3),\] where $r_u=\max\{r_u^1,r_u^2,\dots, r_u^{n_u}\}$,  $\forall u \in [3]$.
\end{definition}


\begin{lemma}\label{lem:equ} \cite{KM11}
	Suppose that ${\mathcal A_u}, {\mathcal B_u}$ are arbitrary tensors. Let ${\mathcal F_u} = {\mathcal A_u}{ \ast _u}{\mathcal B_u}$. Then, the following properties hold	
	\begin{enumerate}
		\item $\left\| {\mathcal A} \right\|_F^2 = \frac{1}{{{n_u}}}\left\| {{{\bar A}_u}} \right\|_F^2$;
		\item ${\mathcal F_u} = {\mathcal A_u}{ \ast _u}{\mathcal B_u}$ and ${{\bar F}_u} = {{\bar A}_u}{{\bar B}_u}$ are equivalent.	
	\end{enumerate}		
\end{lemma}
From above result, we can assert that the tensor factorization can be obtained by matrix factorization, which is computable.

In fact, Generalized $\bm{T}_u$-product and Multi-tubal rank vector reduces to classic $T$-product and tubal rank respectively \cite{KM11} when $u$ is fixed as $3$.








\iffalse
Clearly, $r_3$ is the tubal rank of tensor $\A$ in \cite{KM11} and hence we call the vector of ranks multi-tubal rank in this paper.



Generalized  $\bm{T}_u$-product reduces to classic $\bm{T}$-product when $u$ is fixed as $3$.




\begin{lemma}\label{lemma2.1} \citeonline{KM11} 
Suppose that ${\mathcal A_j}, {\mathcal B_j}$ are two arbitrary tensors. Let ${\mathcal F_j} = {\mathcal A_j}{ \times _j}{\mathcal B_j}$. Then,the following properties hold	
\begin{enumerate}
\item $\left\| {\mathcal A} \right\|_F^2 = \frac{1}{{{n_j}}}\left\| {{{\bar A}_j}} \right\|_F^2$;
\item ${\mathcal F_j} = {\mathcal A_j}{ \times _j}{\mathcal B_j}$ and ${{\bar F}_j} = {{\bar A}_j}{{\bar B}_j}$ are equivalent.	
\end{enumerate}		
\end{lemma}
Note that by utilizing Lemma\ref{lemma2.1} , we can compute $ T_j $-SVD
in an efficient way. We know that \eqref{gs2.1} is equivalent to ${{\bar A}_j} = {{\bar U}_j}{{\bar S}_j}\bar V_j^*(j = 1,2,3)$, where $\bar A_j^{(i)} = \bar U_j^{(i)}\bar S_j^{(i)}{\left( {\bar V_j^{(i)}} \right)^*}$ is the SVD of $\bar A_j^{(i)}$, in which $\bar U_j^{(i)},\bar S_j^{(i)}$ and ${\bar V_j^{(i)}}$ are the $ i $-th horizontal(lateral , frontal) slices of $\bar {\mathcal U},\bar {\mathcal S}$ and $\bar {\mathcal V}$, respectively. Thus, we can compute the SVD of $\bar A_j^{(i)}(j = 1,2,3,i = 1, \cdots ,{n_j})$ to obtain the $  T_j $-SVD of $ {\mathcal A}$. However, computing $ T_j $-SVD is still very computationally expensive.

\fi


==> Chapter/section3.tex <==
\section{TENSOR FACTORIZATION FOR LOW-RANK TENSOR COMPLETION}
In this section, we first present the details of our low-rank tensor
factorization method, and then introduce its optimization and
analyze its convergence. After that, a rank-decreasing method
is proposed to estimate the true rank of a tensor. Finally, we
compare our method with prior work.

\subsection{Formulation of Tensor Factorization}
The  Tensor completion problem can be written as:
\begin{equation}\label{mt-vector}
\mathop {\min }\limits_{{\mathcal C} \in {{\mathbb R}^{{n_1} \times {n_2} \times {n_3}}}} rank_{mt}({\mathcal C}),\quad s.t.\, {P_\Omega }\left( {{\mathcal C} - {\mathcal M}} \right) = 0.
\end{equation}
 Note that problem \eqref{mt-vector} is a vector optimization, which is hard to solve. For simplicity, we consider the following problem
\begin{equation}\label{mt-scalar}
\mathop {\min }\limits_{\mathcal{C} \in {\mathbb{R}^{{n_1} \times {n_2} \times {n_3}}}} \sum\limits_{u = 1}^3 {{\alpha _u}{r_u}(\mathcal{C})} ,\quad s.t.{\mkern 1mu} {P_\Omega }\left( {\mathcal{C} - \mathcal{M}} \right) = 0.
\end{equation}
where $\alpha_1,\alpha_2,\alpha_3\geq 0$ and $\sum\nolimits_{u = 1}^3 {{\alpha _u}}=1 $.
For a given tensor $\C$, we hope to find low rank tensors $\X_u,\Y_u$ such that $\C$ can be represented by $\X_u\ast_u \Y_u$ for $u \in [3]$. To this end, we find a best low rank approximation of $\C$, which can be factorized as $\X_u, \Y_u$ such that $\C=\X_u\ast_u \Y_u$ for all $u \in [3]$.  Motivated by this, we consider a convex Frobenius norm relaxation model for problem \eqref{mt-scalar}
\begin{equation}\label{mt-tensor-xy}
\mathop {\min }\limits_{{{\mathcal X}_u},{{\mathcal Y}_u}} \sum\limits_{u = 1}^3 {\frac{{{\alpha _u}}}{2}\left\| {{P_\Omega }\left( {{{\mathcal X}_u}{ \times _u}{{\mathcal Y}_u} - {\mathcal M}} \right)} \right\|_F^2}.
\end{equation}
To make problem \eqref{mt-tensor-xy} easy to deal, an auxiliary tensor  $\C$ is introduced  and hence \eqref{mt-tensor-xy} can be rewritten as
\begin{equation}\label{mt-tensor-xyc}
\mathop {\min }\limits_{{{\mathcal X}_u},{{\mathcal Y}_u},{\mathcal C}} \sum\limits_{u= 1}^3 {\frac{{{\alpha _u}}}{2}\left\| {{{\mathcal X}_u}{ \times _u}{{\mathcal Y}_u} - {\mathcal C}} \right\|_F^2} \quad s.t.\, {P_\Omega }\left( {{\mathcal C} - {\mathcal M}} \right) = 0.
\end{equation}
From Lemma \ref{lem:equ}, $\|\X_u\ast_u \Y_u-\C\|_F^2=\frac{1}{n_u}\|\bar X_u\bar Y_u-\bar C_u\|_F^2$ and hence problem (\ref{mt-tensor-xyc}) is equivalent to 
\begin{equation}\label{mt-matrix}
\mathop {\min\limits_{X_u,Y_u,\C}} \sum\limits_{u= 1}^3 {\frac{{{\alpha _u}}}{2n_u}\left\| {\bar X_u \bar Y_u - \bar C_u} \right\|_F^2} \quad s.t.\, {P_\Omega }\left( {{\C} - {\M}} \right) = 0.
\end{equation}
In the following, we present the details of computation of problem \eqref{mt-matrix}. Note $(\bar X_1,\bar Y_1), (\bar X_2,\bar Y_2), (\bar X_3,\bar Y_3)$ are independent, we compute $\C, (\bar X_1,\bar Y_1), (\bar X_2,\bar Y_2), (\bar X_3,\bar Y_3)$ sequentially. By similar analysis in \cite{ZLLZ18}, problem \eqref{mt-matrix} is equivalent to
\begin{equation}\label{mt-finally}
\begin{aligned}
&\mathop {\min} \limits_{{{\hat X}_u},{{\hat Y}_u},{\mathcal C}} \sum\limits_{u = 1}^3 {\frac{\alpha _u}{{2{n_u}}}\sum\limits_{l = 1}^{{n_u}} {\left\| {\hat X_u^{(l)}\hat Y_u^{(l)} - \bar C_u^{(l)}} \right\|_F^2} }   =   \sum\limits_{u = 1}^3 {\sum\limits_{l = 1}^{{n_u}} {\frac{\alpha _u}{{2{n_u}}}\left\| {\hat X_u^{(l)}\hat Y_u^{(l)} - \bar C_u^{(l)}} \right\|_F^2} },  \\
& \, \:\; s.t. \quad {P_\Omega }({\mathcal C} - {\mathcal M}) = 0.
\end{aligned}
\end{equation}







\iffalse
Assume that $ rank_{mt}(\A)=(r_1,r_2,r_3) $. Thus, ${\bar C_u^{(u_l)}}$ can be factorized into the product of two matrices $ \hat X_u^{(u_l)} $ and $ \hat Y_u^{(u_l)} $ of smaller sizes, where $ \hat X_u^{(u_l)} $ and $ \hat Y_u^{(u_l)} $ are the $ u_l $-th block diagonal matrices of $ \hat X_u $ and $ \hat Y_u $, respectively.






there exist block diagonal matrices $\hat X_u, \hat Y_u$ $(u \in [3])$ with $\hat X_u^{i}\in \mathbb{C}^{n_u\times r_u^i} $, $\hat Y_u^{i}\in \mathbb{C}^{n_u\times r_u^i} $



$\bar C$ can be factorized into the product of two matrices $ \hat X_u^{(i)} $ and $ \hat Y_u^{(i)} $ of smaller sizes, where $ \hat X_j^{(i)} $ and $ \hat Y_j^{(i)} $ are the $ i $-th block diagonal matrices of $ \hat X_j $ and $ \hat Y_j $, respectively. Assume that $rank_m^j\left( {\mathcal C} \right) = {r^j}$ and $rank_t^j\left( {\mathcal C} \right) = {{\hat r}^j}$, where $r_i^j = rank\left( {\bar C_j^{(i)}} \right)$ and ${{\hat r}^j} = \max (r_1^j,r_2^j, \cdots ,r_{{n_j}}^j)$.




For fixed $\C$,  ${\bar C_u^{(i_u)}}$ can be factorized into the product of two matrices $ \hat X_j^{(i)} $ and $ \hat Y_j^{(i)} $ of smaller sizes, where $ \hat X_j^{(i)} $ and $ \hat Y_j^{(i)} $ are the $ i $-th block diagonal matrices of $ \hat X_j $ and $ \hat Y_j $, respectively. Assume that $rank_m^j\left( {\mathcal C} \right) = {r^j}$ and $rank_t^j\left( {\mathcal C} \right) = {{\hat r}^j}$, where $r_i^j = rank\left( {\bar C_j^{(i)}} \right)$ and ${{\hat r}^j} = \max (r_1^j,r_2^j, \cdots ,r_{{n_j}}^j)$. Thus, Let
\begin{equation*}
\bar X_{\text{1}}^{(i)} = \left[ {\hat X_{\text{1}}^i,0} \right] \in {C^{{n_{\text{2}}} \times {{\hat r}^1}}},\bar X_{\text{2}}^{(i)} = \left[ {\hat X_{\text{2}}^i,0} \right] \in {C^{{n_1} \times {{\hat r}^2}}},\bar X_{\text{3}}^{(i)} = \left[ {\hat X_{\text{3}}^i,0} \right] \in {C^{{n_1} \times {{\hat r}^3}}}.
\end{equation*}
and
\begin{equation*}
\bar Y_{\text{1}}^{(i)} = \left[ {\hat Y_{\text{1}}^i;0} \right] \in {C^{{{\hat r}^1} \times {n_3}}},\bar Y_{\text{2}}^{(i)} = \left[ {\hat Y_{\text{2}}^i;0} \right] \in {C^{{{\hat r}^2} \times {n_3}}},\bar Y_{\text{3}}^{(i)} = \left[ {\hat Y_{\text{3}}^i;0} \right] \in {C^{{{\hat r}^3} \times {n_2}}}.
\end{equation*}
Then, we have ${{\hat X}_j}{{\hat Y}_j} = {{\bar X}_j}{{\bar Y}_j}$. From Lemma \ref{lemma2.1}, we know that ${{\bar X}_j}{{\bar Y}_j}$ and ${{\mathcal X}_j}{ \times _j}{\mathcal Y}$ are equivalent and $\left\| {{{\mathcal X}_j}{ \times _j}{{\mathcal Y}_j} - {\mathcal C}} \right\|_F^2 = \frac{1}{{{n_j}}}\left\| {{{\bar X}_j}{{\bar Y}_j} - {{\bar C}_j}} \right\|_F^2$. Thus, problem \eqref{gs3.4} is equivalent to
\begin{equation}\label{gs3.5}
\begin{aligned}
&\mathop {\min} \limits_{{{\hat X}_j},{{\hat Y}_j},{\mathcal C}} \sum\limits_{j = 1}^3 {\frac{\alpha _j}{{2{n_j}}}\sum\limits_{i = 1}^{{n_j}} {\left\| {\hat X_j^{(i)}\hat Y_j^{(i)} - \bar C_j^{(i)}} \right\|_F^2} }   =   \sum\limits_{j = 1}^3 {\sum\limits_{i = 1}^{{n_j}} {\frac{\alpha _j}{{2{n_j}}}\left\| {\hat X_j^{(i)}\hat Y_j^{(i)} - \bar C_j^{(i)}} \right\|_F^2} },  \\
& \, \:\; s.t. \quad {P_\Omega }({\mathcal C} - {\mathcal M}) = 0.
\end{aligned}
\end{equation}










where $ {rank_{t}} (\mathcal{C}) $ denotes the tubal rank of $  \mathcal{C} $ and ${P_\Omega }$ is the linear operator that extracts entries in $ \Omega $ and fills the entries not in $ \Omega $ with zeros. But since minimizing $ {rank_{t}} (\mathcal{C}) $ is complicated, replace $ {rank_{t}} (\mathcal{C}) $ with the convex combination of the ranks of all horizontal slices, Lateral slices and frontal slices of $ \bar {\mathcal C} $, $ i.e. $, $\sum_{j = 1}^3 {\sum_{i = 1}^{{n_j}} {rank} \left( {{{\bar C}^{(i)}}} \right)} $. To make it easier to solve, Zhang et al. \cite{ZEAHK14} used the tensor nuclear norm $\sum_{j = 1}^3 {\sum_{i = 1}^{{n_j}} {{{\left\| {{{\bar C}^{(i)}}} \right\|}_*}} } $ defined in Definition \ref{definition2.7} to approximate the rank function, and obtained the latest completed results \cite{ZEAHK14}. However, the tensor nuclear norm problem involves SVD every iteration. To make matters worse, tensor data is usually very large. Therefore, this method of minimizing the kernel norm has a high computational cost for multiple SVDs. Since the low-rank matrix decomposition method can more effectively process large-scale data \cite{WYZ12}, we use the low-rank tensor decomposition method to recover the low-rank tensor, aiming to find a faster tensor completion method. We first give two properties of rank of tensor tubal rank in lemma \ref{lemma3.1}
\begin{lemma}\label{lemma3.1} 
Suppose that $ \mathcal F_j $, $ \mathcal A_j $ and $ \mathcal B_j $ are three arbitrary tensors. Then the following properties hold
\begin{enumerate}
	\item If $rank_t^j({\mathcal F_j}) = k$, then $ \mathcal F_j $ can be written into a tensor product form ${\mathcal F_j} = {\mathcal G_j}{ \times _j}{\mathcal H_j}$, where $ \mathcal G_j $ and $ \mathcal H_j $ are two tensors of smaller sizes with $rank_t^j({{\mathcal G}_j}) = rank_t^j({{\mathcal H}_j}) = {k_j}$;	
	\item 	$rank_t^j({{\mathcal A}_j}{ \times _j}{{\mathcal B}_j}) \leqslant \min \left( {rank_t^j{{\mathcal A}_j},rank_t^j{{\mathcal B}_j}} \right)$.
\end{enumerate}	
\end{lemma}
Using Lemma \ref{lemma3.1}, we can factorize any tensor $ \mathcal M_j $ of a tensor tubal rank $ r_j $ as the tensor product form ${\mathcal M_j} = {\mathcal X_j}{ \times _j}{\mathcal Y_j}$, while $rank_t^j({{\mathcal X}_j}) = rank_t^j({{\mathcal Y}_j}) = {k_j}$. Thus, we can control the rank of the tensor $ \mathcal M_j $ by controlling the sizes of two tensors $ \mathcal X_j $ and $ \mathcal Y_j $. Therefore, updating and storing two smaller tensors can be more efficient. At the same time, following most tensor completion methods \cite{XHYS13,LS13,WYZ12}, the noise in the observation data is assumed to be Gaussian observation noise, which is characterized by the Frobenius norm. Accordingly, our tensor completion model can be written as:
\begin{equation}\label{1}
\mathop {\min }\limits_{{{\mathcal X}_j},{{\mathcal Y}_j}} \sum\limits_{j = 1}^3 {\frac{{{\alpha _j}}}{2}\left\| {{P_\Omega }\left( {{{\mathcal X}_j}{ \times _j}{{\mathcal Y}_j} - {\mathcal M}} \right)} \right\|_F^2}. 
\end{equation}
where:$ \sum\nolimits_{j = 1}^3 {{\alpha _j}}  = 1 $. In order to solve problem \eqref{1} more conveniently, we introduce an auxiliary variable $ \mathcal C $ and rewrite problem \eqref{1} as follows:
\begin{equation}\label{gs3.4}
\mathop {\min }\limits_{{{\mathcal X}_j},{{\mathcal Y}_j},{\mathcal C}} \sum\limits_{j = 1}^3 {\frac{{{\alpha _j}}}{2}\left\| {{{\mathcal X}_j}{ \times _j}{{\mathcal Y}_j} - {\mathcal C}} \right\|_F^2} \quad s.t.\, {P_\Omega }\left( {{\mathcal C} - {\mathcal M}} \right) = 0.
\end{equation}
Now, we discuss problem \eqref{gs3.4} in detail. Assume that $rank_m^j\left( {\mathcal C} \right) = {r^j}$ and $rank_t^j\left( {\mathcal C} \right) = {{\hat r}^j}$, where $r_i^j = rank\left( {\bar C_j^{(i)}} \right)$ and ${{\hat r}^j} = \max (r_1^j,r_2^j, \cdots ,r_{{n_j}}^j)$. Thus, ${\bar C_j^{(i)}}$ can be factorized into the product of two matrices $ \hat X_j^{(i)} $ and $ \hat Y_j^{(i)} $ of smaller sizes, where $ \hat X_j^{(i)} $ and $ \hat Y_j^{(i)} $ are the $ i $-th block diagonal matrices of $ \hat X_j $ and $ \hat Y_j $，, respectively. Let 
\begin{equation*}
\bar X_{\text{1}}^{(i)} = \left[ {\hat X_{\text{1}}^i,0} \right] \in {C^{{n_{\text{2}}} \times {{\hat r}^1}}},\bar X_{\text{2}}^{(i)} = \left[ {\hat X_{\text{2}}^i,0} \right] \in {C^{{n_1} \times {{\hat r}^2}}},\bar X_{\text{3}}^{(i)} = \left[ {\hat X_{\text{3}}^i,0} \right] \in {C^{{n_1} \times {{\hat r}^3}}}.
\end{equation*}
and 
\begin{equation*}
\bar Y_{\text{1}}^{(i)} = \left[ {\hat Y_{\text{1}}^i;0} \right] \in {C^{{{\hat r}^1} \times {n_3}}},\bar Y_{\text{2}}^{(i)} = \left[ {\hat Y_{\text{2}}^i;0} \right] \in {C^{{{\hat r}^2} \times {n_3}}},\bar Y_{\text{3}}^{(i)} = \left[ {\hat Y_{\text{3}}^i;0} \right] \in {C^{{{\hat r}^3} \times {n_2}}}.
\end{equation*}
Then, we have ${{\hat X}_j}{{\hat Y}_j} = {{\bar X}_j}{{\bar Y}_j}$. From Lemma \ref{lemma2.1}, we know that ${{\bar X}_j}{{\bar Y}_j}$ and ${{\mathcal X}_j}{ \times _j}{\mathcal Y}$ are equivalent and $\left\| {{{\mathcal X}_j}{ \times _j}{{\mathcal Y}_j} - {\mathcal C}} \right\|_F^2 = \frac{1}{{{n_j}}}\left\| {{{\bar X}_j}{{\bar Y}_j} - {{\bar C}_j}} \right\|_F^2$. Thus, problem \eqref{gs3.4} is equivalent to
\begin{equation}\label{gs3.5}
\begin{aligned}
&\mathop {\min} \limits_{{{\hat X}_j},{{\hat Y}_j},{\mathcal C}} \sum\limits_{j = 1}^3 {\frac{\alpha _j}{{2{n_j}}}\sum\limits_{i = 1}^{{n_j}} {\left\| {\hat X_j^{(i)}\hat Y_j^{(i)} - \bar C_j^{(i)}} \right\|_F^2} }   =   \sum\limits_{j = 1}^3 {\sum\limits_{i = 1}^{{n_j}} {\frac{\alpha _j}{{2{n_j}}}\left\| {\hat X_j^{(i)}\hat Y_j^{(i)} - \bar C_j^{(i)}} \right\|_F^2} },  \\
& \, \:\; s.t. \quad {P_\Omega }({\mathcal C} - {\mathcal M}) = 0.
\end{aligned}
\end{equation}
\fi






\subsection{Optimization of Tensor Factorization}
Problem \eqref{mt-finally} is not jointly convex with respect to $\left( {{{\hat X}_u},{{\hat Y}_u},\mathcal C} \right)(u \in [3])$. Empirically, we can develop an iterative minimization method to update each variable alternately. Similar to \cite{XHYS13,WYZ12} which respectively use the alternating minimization algorithm to optimize matrix and tensor completion problem, here we also adopt it as our optimization method. We can update the three variables in turn as follows:

\begin{itemize}
\item For $ \mathcal C $-subproblem. 
Fix $ \hat X_u (u \in [3]) $ and $ \hat Y_u (u \in [3]) $, we obtain $ \mathcal C $ by solving  
\begin{equation}\label{opt-c}
\begin{aligned}
{\mathcal C} = \mathop {\operatorname{argmin} }\limits_{{P_\Omega }({\mathcal C} - {\mathcal M}) = 0} \frac{1}{2}\sum\limits_{u = 1}^3 {{\alpha _u}\left\| {{{\mathcal X}_u} { \ast _u} {{\mathcal Y}_u} - {\mathcal C}} \right\|_F^2}.
\end{aligned}
\end{equation}
In the following, we will discuss how to solve \eqref{opt-c}. Before this, we need a Lemma.
\begin{lemma}\label{lem:equ-c}
\begin{equation*}
\begin{aligned}
 \mathop {\operatorname{argmin} }\limits_{{P_\Omega }({\mathcal C} - {\mathcal M}) = 0} \frac{1}{2}\sum\limits_{u = 1}^3 {{\alpha _u}\left\| {{{\mathcal X}_u} { \ast _u} {{\mathcal Y}_u} - {\mathcal C}} \right\|_F^2}  = \mathop {\operatorname{argmin} }\limits_{{P_\Omega }({\mathcal C} - {\mathcal M}) = 0} \frac{1}{2}\left\| {\sum\limits_{u = 1}^3 {{\alpha _u}{{\mathcal X}_u} { \ast _u} {{\mathcal Y}_u}}  - {\mathcal C}} \right\|_F^2.
\end{aligned}
\end{equation*}		
\end{lemma}

\begin{proof}
	because
\begin{equation*}
\begin{aligned}
&\quad \sum\limits_{u = 1}^3 {{\alpha _u}\left\| {{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u} - \mathcal{C}} \right\|_F^2}  
= \sum\limits_{u = 1}^3 {{\alpha _u}\left\langle {{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u} - \mathcal{C},{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u} - \mathcal{C}} \right\rangle }   \\
&= \sum\limits_{u = 1}^3 {{\alpha _u}\left\langle {\mathcal{C},\mathcal{C}} \right\rangle }  - 2\sum\limits_{u = 1}^3 {{\alpha _u}\left\langle {{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u},\mathcal{C}} \right\rangle }  + \sum\limits_{u = 1}^3 {{\alpha _u}\left\langle {{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u},{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u}} \right\rangle }   \\
&= \left\langle {\mathcal{C},\mathcal{C}} \right\rangle  - 2\left\langle {\sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u}} ,\mathcal{C}} \right\rangle  + \sum\limits_{u = 1}^3 {{\alpha _u}\left\| {{\mathcal{X}_u}{ \ast _u}\mathcal{Y}} \right\|_F^2}   \\
&= \left\langle {\sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u}}  - \mathcal{C},\sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u}}  - \mathcal{C}} \right\rangle  + \sum\limits_{u = 1}^3 {{\alpha _u}\left\| {{\mathcal{X}_u}{ \ast _u}\mathcal{Y}} \right\|_F^2}  - \left\| {\sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u}} } \right\|_F^2  \\
&= \left\| {\sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}*{\mathcal{Y}_u}}  - \mathcal{C}} \right\|_F^2 + \sum\limits_{u = 1}^3 {{\alpha _u}\left\| {{\mathcal{X}_u}{ \ast _u}\mathcal{Y}} \right\|_F^2}  - \left\| {\sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u}} } \right\|_F^2. 
\end{aligned}
\end{equation*}
and $ \sum\limits_{u = 1}^3 {{\alpha _u}\left\| {{\mathcal{X}_u}{ \ast _u}\mathcal{Y}} \right\|_F^2}  - \left\| {\sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u}} } \right\|_F^2 $ is constant, so
\begin{equation*}
\begin{aligned}
\mathop {\operatorname{argmin} }\limits_{{P_\Omega }({\mathcal C} - {\mathcal M}) = 0} \frac{1}{2}\sum\limits_{u = 1}^3 {{\alpha _u}\left\| {{{\mathcal X}_u} { \ast _u} {{\mathcal Y}_u} - {\mathcal C}} \right\|_F^2}  = \mathop {\operatorname{argmin} }\limits_{{P_\Omega }({\mathcal C} - {\mathcal M}) = 0} \frac{1}{2}\left\| {\sum\limits_{u = 1}^3 {{\alpha _u}{{\mathcal X}_u} { \ast _u} {{\mathcal Y}_u}}  - {\mathcal C}} \right\|_F^2.
\end{aligned}
\end{equation*}	
\end{proof}
Knowing from Lemma \ref{lem:equ-c}, the solution of \eqref{opt-c} is
\begin{equation}\label{opt-c-solution}
\begin{aligned}
\mathcal{C} &= \mathop {\operatorname{argmin} }\limits_{{P_\Omega }(\mathcal{C} - \mathcal{M}) = 0} \frac{1}{2}\sum\limits_{u = 1}^3 {{\alpha _u}\left\| {{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u} - \mathcal{C}} \right\|_F^2}  \hfill \\
&= \mathop {\operatorname{argmin} }\limits_{{P_\Omega }(\mathcal{C} - \mathcal{M}) = 0} \frac{1}{2}\left\| {\sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u}}  - \mathcal{C}} \right\|_F^2 \hfill \\
&= \sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u}}  + {P_\Omega }\left( {\mathcal{M} - \sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _u}{\mathcal{Y}_u}} } \right). \hfill \\ 
\end{aligned}
\end{equation}



\item  For $ \hat X_u  $-subproblem. 
Fix $ \mathcal C $ and $ \hat Y_u (u \in [3]) $, we obtain $ \hat X_u  $ by solving
\begin{equation}\label{opt-x}
\begin{aligned}
\hat X_u^{(l)} &= \mathop {\operatorname{argmin} }\limits_{\hat X_u^{(l)}} \frac{1}{{2{n_u}}}\left\| {\hat X_u^{(l)}\hat Y_u^{(l)} - \bar C_u^{(l)}} \right\|_F^2 
\\&= \bar C_u^{(l)}{\left( {\hat Y_u^{(l)}} \right)^*}{\left( {\hat Y_u^{(l)}{{\left( {\hat Y_u^{(l)}} \right)}^*}} \right)^\dag } \quad  u \in [3] ,  l \in [n_u].
\end{aligned}
\end{equation}

\item  For $ \hat Y_u  $-subproblem. 
Fix $ \mathcal C $ and $ \hat X_u (u \in [3]) $, we obtain $ \hat Y_u  $ by solving
\begin{equation}\label{opt-y}
\begin{aligned}
\hat Y_u^{(l)} &= \mathop {\operatorname{argmin} }\limits_{\hat Y_u^{(l)}} \frac{1}{{2{n_u}}}\left\| {\hat X_u^{(l)}\hat Y_u^{(l)} - \bar C_u^{(l)}} \right\|_F^2 
\\&= {\left( {{{\left( {\hat X_u^{(l)}} \right)}^*\hat X_u^{(l)}}} \right)^\dag }{\left( {\hat X_u^{(l)}} \right)^*}\bar C_u^{(l)} \quad  u \in [3] ,  l \in [n_u].
\end{aligned}
\end{equation}
\end{itemize}

After updating $\hat X_u^{l}$ and $ \hat Y_u^{l}$, we can compute ${{\mathcal X}_u}{ \ast _u}{{\mathcal Y}_u}$ in an efficient way. 
Assume that $\mathcal G =\sum\limits_{u = 1}^3 {{\alpha _u}{{\mathcal X}_u} { \ast _j} {{\mathcal Y}_u}} $. Then we first compute $\bar G_u^{(l)} = \hat X_u^{(l)}\hat Y_u^{(l)}(u \in [3],l \in [n_j])$ and obtain
$${\mathcal G} = \sum\limits_{u = 1}^3 {\alpha_j*ifft({{\bar G}_u},[],u)}. $$
This is more efficient than directly computing $\mathcal C =\sum\limits_{u = 1}^3 {{\alpha _u}{{\mathcal X}_u} { \ast _j} {{\mathcal Y}_u}} $.The detailed optimization procedure is presented in Algorithm 1.

\begin{remark}
 since equations \eqref{opt-x},\eqref{opt-y} are ill-conditioned and may be singular, To enforce the positive definiteness of the subproblems, Navasca et al. \cite{NDK08,LKN13} propose to add a regularization
term to the subproblem and minimize.

\begin{equation}\label{opt-x-reg}
\begin{aligned}
\hat X_u^{(l)} &= \mathop {\operatorname{argmin} }\limits_{\hat X_u^{(l)}} \frac{1}{{2{n_u}}}\left\| {\hat X_u^{(l)}\hat Y_u^{(l)} - \bar C_u^{(l)}} \right\|_F^2 + \frac{\lambda }{{2{n_u}}}\left\| {\hat X_u^{(l)}} \right\|_F^2   \\
&= \bar C_u^{(l)}{\left( {\hat Y_u^{(l)}} \right)^*}{\left( {\hat Y_u^{(l)}{{\left( {\hat Y_u^{(l)}} \right)}^*} + \lambda I} \right)^{ - 1}}\quad u \in [3] ,  l \in [n_u].
\end{aligned}
\end{equation}

\begin{equation}\label{opt-y-reg}
\begin{aligned}
\hat Y_u^{(l)} &= \mathop {\operatorname{argmin} }\limits_{\hat Y_u^{(l)}} \frac{1}{{2{n_u}}}\left\| {\hat X_u^{(l)}\hat Y_u^{(l)} - \bar C_u^{(l)}} \right\|_F^2 + \frac{\lambda }{{2{n_u}}}\left\| {\hat Y_u^{(l)}} \right\|_F^2 
\\&= {\left( {{{\left( {\hat X_u^{(l)}} \right)}^*}\hat X_u^{(l)} + \lambda I} \right)^{ - 1}}{\left( {\hat X_u^{(l)}} \right)^*}\bar C_u^{(l)}\quad u \in [3] ,  l \in [n_u].
\end{aligned}
\end{equation}

Note that the regularized parameter µk should decrease monotonically as iterations process. A classical strategy for choosing µk is the geometric sequence \cite{DH13,DNR12}. In this paper, To achieve rapid convergence, we choice for the parameter sequence $ lamda $ is the geometric sequence
$${\lambda _n} = {\lambda _0}{q^n},n = 1,2, \cdots. $$
where $ \lambda _0 > 0 $ and $ 0 < q \leqslant 1. $ The  stationary iterated  method is obtained for $ q = 1 $. 
\end{remark}
\par Hence, based on the above discussions, we propose the tensor Completion by Tensor Factorization method for solving problem \eqref{mt-finally} as follows.

\begin{table}[htbp]
	\centering
	% \begin{center}   
	\begin{tabular}{l}
		\toprule 
		\toprule
         {\bfseries Algorithm 1} Tensor Completion by Tensor Factorization Group(TCTFG)       \\    
		\midrule
		{\bfseries Input:}The tensor data ${\mathcal M} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$, the observed set  
		$\Omega $, the initialized \\ rank $ R^0 ,\lambda_0,q$, and $ \epsilon=1e-5 $.                                  \\
		{\bfseries Initialize: } $\hat X_u^0,\hat Y_u^0,j \in [3]$.                                           \\
		{\bfseries While not converge do}                \\
		\qquad  \bm{1.} Fix $\hat X_u^k$ and $ \hat Y_u^k $ to update $\mathcal C^{k+1} $ by \eqref{opt-c-solution}, and then
		compute  $\bar C$.                                \\
		\qquad  \bm{2.} Fix $\hat Y_u^k$ and $\mathcal C^{k+1} $ to update $\hat X_u^{k+1}$ by \eqref{opt-x-reg}.     \\
		\qquad  \bm{3.} Fix $\hat X_u^{k+1}$ and $\mathcal C^{k+1} $ to update $\hat Y_u^{k+1}$ by \eqref{opt-y-reg}.     \\
		\qquad  \bm{4.} Adopt the rank decreasing scheme  to adjust $ rank_{mt}(\A) $ and  the sizes \\ \qquad  of  $\hat X_u^{k+1}$ and $ \hat Y_u^{k+1} $. \\
		\qquad  \bm{5.} Check the convergence condition:${\left\| {\hat X_u^{k + 1} - \hat X_u^k} \right\|_\infty } < \varepsilon ,{\left\| {\hat Y_u^{k + 1} - \hat Y_u^k} \right\|_\infty } $  \\
		\qquad $< \varepsilon ,{\left\| {{\mathcal C^{k + 1}} - {\mathcal C^k}} \right\|_\infty } < \varepsilon $.  \\
		\qquad  \bm{6.} $k \leftarrow k + 1$,$ {\lambda _{k+1}} = {\lambda _k}{q^n} $.            \\
		{\bfseries end while}                             \\
		{\bfseries Output:} $\hat X_u^{k+1},\hat Y_u^{k+1}$, and $\mathcal C^{k + 1}  $.      \\		
		 \bottomrule 
		 \bottomrule
	\end{tabular}
	% \end{center}
\end{table}


\subsection{Improvement with Spatio-Temporal}
In actual data, some data usually changes slowly over time, and these data show time stability in the time dimension. For example, the data between two adjacent frames of the video, the traffic data of two adjacent days, and so on.
\par To capture these domain knowledge, we introduce more regularization terms into the optimization objective. we propose to
combine with \eqref{mt-finally} and solve the following
\begin{equation}\label{mt-st}
\begin{aligned}
&\mathop {\min }\limits_{{{\mathcal X}_u},{{\mathcal Y}_u},{\mathcal C}} \sum\limits_{u = 1}^3 {\frac{{{\alpha _u}}}{2}\left\| {{{\mathcal X}_u}{ \ast _u}{{\mathcal Y}_u} - {\mathcal C}} \right\|_F^2}+\frac{\beta }{2}\sum\limits_{u = 1}^3 {\left\| {{T_u} \cdot unfol{d_u}({\mathcal C})} \right\|_F^2}, \\
&\;\;s.t.\,{P_\Omega }\left( {{\mathcal C} - {\mathcal M}} \right) = 0.
\end{aligned}
\end{equation}
where $ unfold_u({{\mathcal C}}) = [C_u^{(1)};C_u^{(2)}; \cdots ;C_u^{({n_u})}] $, $ T_{1} $ and $ T_{2} $ are the spatial constraint matrices and $ T_{3} $ is the temporal constraint matrix, which expresses our knowledge about the data spatio-temporal properties. The temporal constraint $ T_{3} $ captures temporal stability feature, i.e., the data is similar at adjacent time slots in the tensor. Based on $ unfold{_3}({\mathcal C}) $, we set $ T_{3} = Toeplitz(0; I; −I) $ of the size $ (n_{3}-1) \times n_{3} $ , which denotes the Toeplitz matrix with central diagonal given by $ I $, the first upper diagonal given by $ -1 $, and the others given by $ 0 $, i.e.,
\begin{align*}
T_{3}=\left[\begin{array}{cccc}
I & -I & 0 & \cdots \\
0 & I & -I & \ddots \\
0 & 0 & I & \ddots \\
\vdots & \ddots & \ddots & \ddots
\end{array}\right]
\end{align*}
The  matrix $ \mathcal C_3^{(k)} $ is the principal components in time
dimension of tensor, i.e., temporal lower-dimensional representation. By minimizing 
$$ \left\| {{T_3}\cdot unfol{d_3}(C)} \right\|_F^2=\sum\limits_{k = 1}^{{n_3} - 1} \left\| {\mathcal{C}_{\text{3}}^{^{(k)}} - \mathcal{C}_{\text{3}}^{^{(k + 1)}}} \right\|_F^2. $$
 The temporal constraint $ T_{3} $ functions on the latent space of time dimension of tensor, which approximate the property of having similar values at adjacent time slots.
\par The spatial constraint $ T_{1} $ and $ T_{2} $ capture spatial correlation feature, i.e., the data is similar in spatial dimension of
tensor. Using $ unfold{_1}({\mathcal C}) $ and $ unfold{_2}({\mathcal C}) $, we chose $ T_{1} $ and $ T_{2} $ based on the similarity between $ \mathcal C_1^{(i)} $ and $ \mathcal C_1^{(j)}(j \ne i) $, $ \mathcal C_2^{(i)} $ and $ \mathcal C_2^{(j)}(j \ne i) $ respectively. For each $ \mathcal C_1^{(i)} $, we perform linear regression to find a set
of weights $w_{1}(n)(n \in [n_{1}-1])$ such that the linear
combination of $ \mathcal C_1^{(j_{n})} $ best approximates the $ \mathcal C_1^{(i)} $, i.e., $ \mathcal{C}_{\text{1}}^{(i)} = \sum {{w_i}(n)\mathcal{C}_{\text{1}}^{{(j_n)}}}  $. Then we set $ T_{1}(i, i) = I $ and $ T_{1} (i, j_{n}) = -w_{i}(n)I $. For choosing $ T_{2} $, the entire procedure is repeated using $ unfold{_2}({\mathcal C}) $. The matrices $ T_{1} $ and $ T_{2} $ express spatial similar relationship of data. As the matrices $ unfold{_1}({\mathcal C}) $ and $ unfold{_2}({\mathcal C}) $ are lowerdimensional representation of the spatial dimension, by minimizing 
\[\left\| {{T_1}\cdot unfol{d_1}(C)} \right\|_F^2 = \sum\limits_{i = 1}^{{n_1}} {\left\| {C_1^{(i)} - \sum\limits_{j \ne i} {{w_i}(j)C_1^{(j)}} } \right\|} _F^2\]
and
\[\left\| {{T_2}\cdot unfol{d_2}(C)} \right\|_F^2 = \sum\limits_{i = 1}^{{n_2}} {\left\| {C_2^{(i)} - \sum\limits_{j \ne i} {{w_i}(j)C_2^{(j)}} } \right\|} _F^2.\]
the spatial constraint $ T_{1} $ and $ T_{2} $ function on the underlying latent structure of spatial dimension, which approximate spatial correlation feature.
\par To find $ T_{u} (u \in [2]) $, we are obliged to estimate an initial
traffic tensor $ \hat {\mathcal C} $ without missing data and outlier because these factors may destroy spatial feature. One way is to first
run once, which only utilizes the temporal constraint
(i.e., $ T_{3} $) to recover the missing entries and remove outlier.
With initial estimation tensor $ \hat {\mathcal C} $, we analyze the similarities  and perform linear regression to find spatial
constraints (i.e.,$  T_{1}, T_{2} $). At the second run, the learned
$  T_{1}, T_{2} $ and $ T_{3} $ are incorporated into ST-TCTFG to recovery the missing data and remove outlier.
\par Compared with the original problem, the solution method of $ \mathcal{C} $ is mainly changed, and the rest is unchanged. Next consider how to solve $ \mathcal{C} $. In order to solve $ \mathcal{C} $, we need to solve $ unfold_u({{\mathcal C}})(u \in [3]) $, and then let
\begin{align}\label{opt-c-st}
\mathcal{C}=\frac{1}{3}\left( {fold}_{u}\left( {unfold}_{u}(\mathcal{C})\right)\right).
\end{align}
\par From Lemma \ref{lem:equ-c} we know that equation \eqref{opt-c-st} is equivalent to
\begin{equation}\label{opt-c-st-equ}
\begin{aligned}
&\mathop {\min }\limits_\mathcal{C} \frac{1}{2}\left\| {\sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _j}{\mathcal{Y}_u}}  - \mathcal{C}} \right\|_F^2+\frac{\beta }{2}\sum\limits_{u = 1}^3 {\left\| {{T_u} \cdot unfol{d_u}({\mathcal C})} \right\|_F^2}, \\
&\;\;s.t.\,{P_\Omega }\left( {{\mathcal C} - {\mathcal M}} \right) = 0.
\end{aligned}
\end{equation}
Let $ \mathcal{B} = \sum\limits_{u = 1}^3 {{\alpha _u}{\mathcal{X}_u}{ \ast _j}{\mathcal{Y}_u}}  $, then \eqref{opt-c-st-equ} is equivalent to
\begin{equation}\label{c-st}
\begin{aligned}
&\mathop {\min }\limits_\mathcal{C} \frac{1}{2}{\left\| {{\mathcal{B}} - {\mathcal{C}}} \right\|_F^2}  + \frac{\beta }{2}\sum\limits_{u = 1}^3 {\left\| {{T_u} \cdot unfol{d_u}({\mathcal C})} \right\|_F^2}, 
\\&\,\, s.t.\, {P_\Omega }\left( {{\mathcal{C}} - {\mathcal{M}}} \right) = 0.
\end{aligned}
\end{equation}
\par \textbf{Computing $ \bm{unfold_3({{\mathcal C}}):} $} the optimal is the solution to the following subproblem:
\begin{equation}\label{gs3.16}
\begin{aligned}
&\mathop {\min }\limits_{unfold_3({{\mathcal C}})} \frac{1}{2}\sum\limits_{k = 1}^{{n_3}} {\left\| {{\mathcal{B}^{(k)}_3} - {\mathcal{C}^{(k)}_3}} \right\|_F^2}  + \frac{\beta }{2}\sum\limits_{k = 1}^{{n_3} - 1} {\left\| {\mathcal{C}_{\text{3}}^{^{(k)}} - \mathcal{C}_{\text{3}}^{^{(k + 1)}}} \right\|_F^2}, 
\\&\,\, s.t.\, {P_\Omega }\left( {{\mathcal{C}^{(k)}_3} - {\mathcal{M}^{(k)}_3}} \right) = 0,k \in [n_3].
\end{aligned}
\end{equation}


We can update $ {{\mathcal{C}_3^{(k)}}},k \in [n_3]. $ in turn as follows:
\begin{itemize}
\item For $ {{\mathcal{C}^{(1)}_3}} $-subproblem. 
Fix $ {{\mathcal{C}^{(k)}_3}} (k = 2,\dots,n_{3}) $ , we obtain $ {{\mathcal{C}^{(1)}_3}} $ by solving  
\begin{equation}\label{c-st-3-1}
\mathop {\min }\limits_{{\mathcal{C}^{(1)}_3}} \frac{1}{2}\left\| {{\mathcal{B}^{(1)}_3} - {\mathcal{C}^{(1)}_3}} \right\|_F^2 + \frac{\beta }{2}\left\| {{\mathcal{C}^{(1)}_3} - {\mathcal{C}^{(2)}_3}} \right\|_F^2,\quad s.t.\, {P_\Omega }\left( {{\mathcal{C}^{(1)}_3} - {\mathcal{M}^{(1)}_3}} \right) = 0.
\end{equation}	
A proof similar to Lemma \ref{lem:equ-c} shows that \eqref{c-st-3-1} is equivalent to	
\begin{equation}\label{c-st-3-1-equ}
\mathop {\min }\limits_{\mathcal{C}_3^{(1)}} \frac{{1 + \beta }}{2}\left\| {\mathcal{C}_3^{(1)} - \frac{1}{{1 + \beta }}\left( {\mathcal{B}_3^{(1)}+\beta \mathcal{C}_3^{(2)}} \right)} \right\|_F^2,\quad s.t.\, {P_\Omega }\left( {\mathcal{C}_3^{(1)} - \mathcal{M}_3^{(1)}} \right) = 0.
\end{equation}	
It is easy to check that the optimal solution to \eqref{c-st-3-1-equ} is give by
\begin{align}\label{c-st-3-1-solution}
\mathcal{C}^{(1)}_3=\frac{1}{1+\beta}\left(\mathcal{B}_{3}^{(1)}+\beta\mathcal{C}_{3}^{(2)}\right)+P_{\Omega}\left(\mathcal{M}_{3}^{(1)}-\frac{1}{1+\beta}\left(\mathcal{B}_{3}^{(1)}+\beta \mathcal{C}_{3}^{(2)}\right)\right).
\end{align}
	
\item For $ {{\mathcal{C}^{(n_{3})}_3}} $-subproblem. 
Fix $ {{\mathcal{C}^{(k)}_3}} (k = 1,\dots,n_{3}-1) $ , we obtain $ {{\mathcal{C}^{(n_{3})}_3}} $ by solving 
\begin{equation}\label{c-st-3-n3}
\begin{aligned}
&\mathop {\min }\limits_{{\mathcal{C}^{(n_{3})}_3}} \frac{1}{2}\left\| {{\mathcal{B}^{(n_{3})}_3} - {\mathcal{C}^{(n_{3})}_3}} \right\|_F^2 + \frac{\beta }{2}\left\| {{\mathcal{C}^{(n_{3}-1)}_3} - {\mathcal{C}^{(n_{3})}_3}} \right\|_F^2,\\
&\,\,s.t.\, {P_\Omega }\left( {{\mathcal{C}^{(n_{3})}_3} - {\mathcal{M}^{(n_{3})}_3}} \right) = 0.
\end{aligned}
\end{equation}
	
A proof similar to Lemma \ref{lem:equ-c} shows that \eqref{c-st-3-n3} is equivalent to
\begin{equation}\label{c-st-3-n3-equ}
\begin{aligned}
&\mathop {\min }\limits_{\mathcal{C}_3^{(n_{3})}} \frac{{1 + \beta }}{2}\left\| {\mathcal{C}_3^{(n_{3})} - \frac{1}{{1 + \beta }}\left( {\mathcal{B}_3^{(n_{3})}+\beta \mathcal{C}_3^{(n_{3}-1)}} \right)} \right\|_F^2,\\ 
&\,\,s.t.\, {P_\Omega }\left( {\mathcal{C}_3^{(n_{3})} - \mathcal{M}_3^{(n_{3})}} \right) = 0.
\end{aligned}
\end{equation}	
It is easy to check that the optimal solution to \eqref{c-st-3-n3-equ}	is give by
\begin{align}\label{c-st-3-n3-solution}
\mathcal{C}^{(n_{3})}_3=\frac{1}{1+\beta}\left(\mathcal{B}_{3}^{(n_{3})}+\beta\mathcal{C}_{3}^{(n_{3}-1)}\right)+P_{\Omega}\left(\mathcal{M}_{3}^{(n_{3})}-\frac{1}{1+\beta}\left(\mathcal{B}_{3}^{(n_{3})}+\beta \mathcal{C}_{3}^{(n_{3}-1)}\right)\right).
\end{align}	
	
\item For $ {{\mathcal{C}^{(k)}_3}}(k = 2, \cdots ,{n_3}-1) $-subproblem. 
Fix $ {{\mathcal{C}^{(j)}_3}} (j \ne k,j = 1,\dots,n_{3}) $ , we obtain $ {{\mathcal{C}^{(k)}_3}} $ by solving  
\begin{equation}\label{c-st-3-ni}
\begin{aligned}
&\mathop {\min }\limits_{\mathcal{C}_3^{(k)}} \frac{1}{2}\left\| {\mathcal{B}_3^{(k)} - {\mathcal{C}^{(k)}}} \right\|_F^2 + \frac{\beta }{2}\left\| {\mathcal{C}_3^{(k - 1)} - \mathcal{C}_3^{(k)}} \right\|_F^2 + \frac{\beta }{2}\left\| {\mathcal{C}_3^{(k)} - \mathcal{C}_3^{(k + 1)}} \right\|_F^2,  \hfill \\
&\,\,s.t.\, {P_\Omega }\left( {\mathcal{C}_3^{(k)} - \mathcal{M}_3^{(k)}} \right) = 0. \hfill \\ 
\end{aligned}
\end{equation}
A proof similar to Lemma \ref{lem:equ-c} shows that \eqref{c-st-3-ni} is equivalent to
\begin{equation}\label{c-st-3-ni-equ}
\begin{aligned}
&\mathop {\min }\limits_{\mathcal{C}_3^{^{(k)}}} \frac{{1 + 2\beta }}{2}\left\| {\mathcal{C}_3^{^{(k)}} - \frac{1}{{1 + 2\beta }}\left( {\mathcal{B}_3^{^{(k)}}{\text{  +  }}\beta \mathcal{C}_3^{^{(k - 1)}} + \beta \mathcal{C}_3^{^{(k + 1)}}} \right)} \right\|_F^2,  \hfill \\
&\,\, s.t.\, {P_\Omega }\left( {\mathcal{C}_3^{^{(k)}} - \mathcal{M}_3^{^{(k)}}} \right) = 0. \hfill \\ 
\end{aligned}
\end{equation}	
It is easy to check that the optimal solution to \eqref{c-st-3-ni-equ}	is give by
\begin{align}\label{c-st-3-ni-solution}
\mathcal{C}_3^{^{(k)}}{\text{ =  }}\frac{1}{{1 + 2\beta }}\left( {\mathcal{B}_3^{^{(k)}}{\text{  +  }}\beta \mathcal{C}_3^{^{(k - 1)}} + \beta \mathcal{C}_3^{^{(k + 1)}}} \right){\text{  +  }}{P_\Omega }\left( {\mathcal{M}_3^{^{(k)}} - \frac{1}{{1 + 2\beta }}\left( {\mathcal{B}_3^{^{(k)}}{\text{  +  }}\beta \mathcal{C}_3^{^{(k - 1)}} + \beta \mathcal{C}_3^{^{(k + 1)}}} \right)} \right).
\end{align}		
\end{itemize}
In summary, we can Computing $ unfold_3({{\mathcal C}}) $ through \eqref{c-st-3-1-solution}, \eqref{c-st-3-n3-solution} and \eqref{c-st-3-ni-solution}. 

\par \textbf{Computing $ \bm{unfold_1({{\mathcal C}}):} $} the optimal is the solution to the following subproblem:
\begin{equation}\label{c-st-1}
\begin{aligned}
&\mathop {\min }\limits_{unfol{d_1}(C)} \frac{1}{2}\sum\limits_{i = 1}^{{n_1}} {\left\| {\mathcal{B}_1^{(i)} - \mathcal{C}_1^{(i)}} \right\|_F^2}  + \frac{\beta }{2}\left\| {{T_1} \cdot unfold{_1}(\mathcal{C})} \right\|_F^2, 
\\&\,\, s.t.\, {P_\Omega }\left( {{\mathcal{C}_1^{(k)}} - {\mathcal{M}_1^{(k)}}} \right) = 0, i \in [n_{1}].
\end{aligned}
\end{equation}
where 
\[{T_1}\cdot unfold{_1}(\mathcal{C}) = \left( {\begin{array}{*{20}{c}}
	I&{ - {w_1}(2)I}& \cdots &{ - {w_1}({n_1})I} \\ 
	{ - {w_2}(1)I}&I& \cdots &{ - {w_2}({n_1})I} \\ 
	\vdots & \vdots & \ddots & \vdots  \\ 
	{ - {w_{{n_1}}}(1)I}&{ - {w_{{n_1}}}(2)I}& \cdots &I 
	\end{array}} \right)\left( {\begin{array}{*{20}{c}}
	{\mathcal{C}_1^{(1)}} \\ 
	{\mathcal{C}_1^{(2)}} \\ 
	\vdots  \\ 
	{\mathcal{C}_1^{({n_1})}} 
	\end{array}} \right)\]
Therefore, for solving  $ \mathcal{C}_1^{(1)} $, let 
\[\widehat {{T_1}} = \left( {\begin{array}{*{20}{c}}
	1&{ - {w_1}(2)}& \cdots &{ - {w_1}({n_1})} \\ 
	{ - {w_2}(1)}&1& \cdots &{ - {w_2}({n_1})} \\ 
	\vdots & \vdots & \ddots & \vdots  \\ 
	{ - {w_{{n_1}}}(1)}&{ - {w_{{n_1}}}(2)}& \cdots &1 
	\end{array}} \right),C = \left( {\begin{array}{*{20}{c}}
	{\mathcal{C}_1^{(2)}} \\ 
	{\mathcal{C}_1^{(3)}} \\ 
	\vdots  \\ 
	{\mathcal{C}_1^{({n_1})}} 
	\end{array}} \right)\]
and
\[{v_{11}} = \widehat {{T_1}}(1,1),{v_{12}} = \widehat {{T_1}}(1,2:{n_1}),{v_{21}} = \widehat {{T_1}}(2:{n_1},1),{v_{22}} = \widehat {{T_1}}(2:{n_1},2:{n_1}).\]
A proof similar to Lemma \ref{lem:equ-c} we can know
\[\mathcal{C}_1^{(k)} = \frac{{\mathcal{B}_1^{\left( k \right)} - \beta \left( {{v_{11}}{v_{12}} + v_{21}^T{v_{22}}} \right)C}}{{1 + \beta \left( {v_{11}^2 + v_{21}^T{v_{21}}} \right)}}.\]
For solving  $ \mathcal{C}_1^{(k)} $, we only need to exchange the position of the $ i $-th row and the first row of $ \widehat {{T_1}} $ , the $ i $-th matrix and the first matrix of $ unfold{_1}(\mathcal{C}) $, and then follow the solution method of $ \mathcal{C}_1^{(1)} $. Then we can Computing $ unfold_1({{\mathcal C}}) $.
\par \textbf{Computing $ \bm{unfold_2({{\mathcal C}}):} $} Similar to Solving $ unfold_1({{\mathcal C}}) $.
\begin{remark}
\par (1) When we iterate a variable, all other variables are taken as the rank obtained in the previous step;
\par (2) When the data has only time characteristics, we make $ T_{1}= T_{2}= 0 $.
\end{remark}
\par To this end, we introduced improved algorithms, which I call them ST-TCTFG(Algorithm 2).
\begin{table}[htbp]
	\centering
	% \begin{center}   
	\begin{tabular}{l}
		\toprule 
		\toprule
		{\bfseries Algorithm 2} Spatio-Temporal Tensor Completion by Tensor\\ Factorization Group(ST-TCTFG)       \\    
		\midrule
		{\bfseries Input:}The tensor data ${\mathcal M} \in {{\mathbb C}^{{n_1} \times {n_2} \times {n_3}}}$, the observed set  
		$\Omega $, the initialized \\ rank $ R^0 ,\lambda_0,q,T_{3}$, and $ \epsilon=1e-5 $.                                  \\
		{\bfseries Initialize: } $\hat X_u^0,\hat Y_u^0,j \in [3]$.                                           \\
		{\bfseries While not converge do}                \\
		\qquad  \bm{1.} Fix $\hat X_u^k$ and $ \hat Y_u^k $ to update $\mathcal C^{k+1} $ by \eqref{opt-c-st}, and then
		compute  $\bar C$.                                \\
		\qquad  \bm{2.} compute  $ T_{2}$ and $ T_{3}$ in the first step.                                \\
		\qquad  \bm{3.} Fix $\hat Y_u^k$ and $\mathcal C^{k+1} $ to update $\hat X_u^{k+1}$ by \eqref{opt-x-reg}.     \\
		\qquad  \bm{4.} Fix $\hat X_u^{k+1}$ and $\mathcal C^{k+1} $ to update $\hat Y_u^{k+1}$ by \eqref{opt-y-reg}.     \\
		\qquad  \bm{5.} Adopt the rank decreasing scheme to adjust $ rank_{mt}(\A) $ and  the sizes \\ \qquad of  $\hat X_u^{k+1}$ and $ \hat Y_u^{k+1} $. \\
		\qquad  \bm{6.} Check the convergence condition:${\left\| {\hat X_u^{k + 1} - \hat X_u^k} \right\|_\infty } < \varepsilon ,{\left\| {\hat Y_u^{k + 1} - \hat Y_u^k} \right\|_\infty } $  \\
		\qquad $< \varepsilon ,{\left\| {{\mathcal C^{k + 1}} - {\mathcal C^k}} \right\|_\infty } < \varepsilon $.  \\
		\qquad  \bm{7.} $k \leftarrow k + 1$,$ {\lambda _{k+1}} = {\lambda _k}{q^n} $.            \\
		{\bfseries end while}                             \\
		{\bfseries Output:} $\hat X_u^{k+1},\hat Y_u^{k+1}$, and $\mathcal C^{k + 1}  $.      \\		
		\bottomrule 
		\bottomrule
	\end{tabular}
	% \end{center}
\end{table}



\subsection{Convergence Analysis}
By introducing a Lagrange multiplier $\mathcal Q $ so that $\mathcal Q  = {P_\Omega }(\mathcal Q ) $, the Lagrangian function of \eqref{gs3.5} is defined as
\[\mathcal L({{\hat X}_1},{{\hat X}_2},{{\hat X}_3},{{\hat Y}_1},{{\hat Y}_2},{{\hat Y}_3},\mathcal{C},\mathcal Q  ) = \sum\limits_{j = 1}^3 {\frac{{{\alpha _j}}}{{2{n_j}}}\left\| {{{\hat X}_j}{{\hat Y}_j} - {{\bar C}_j}} \right\|_F^2}  + \left\langle {\mathcal Q  ,{P_\Omega }(\mathcal{C} - \mathcal{M})} \right\rangle. \]
Let $ {\nabla _{{{\hat X}_j}}}\mathcal{L} = 0,{\nabla _{{{\hat Y}_j}}}\mathcal{L} = 0 \, (j = 1,2,3),{\nabla _\mathcal{C}}\mathcal{L} = 0,{\nabla _\mathcal{Q}}\mathcal{L} = 0 $. We can obtain the following KKT conditions:
\[\left\{ \begin{gathered}
\left( {{{\hat X}_j}{{\hat Y}_j} - {{\bar C}_j}} \right)\hat Y_j^* = 0, \hfill \\
\hat X_j^*\left( {{{\hat X}_j}{{\hat Y}_j} - {{\bar C}_j}} \right) = 0, \hfill \\
{P_{{\Omega ^C}}}\left( {{C_j} - {\mathcal{X}_j}{ \times _j}{\mathcal{Y}_j}} \right) = 0, \hfill \\
{P_\Omega }(\mathcal{C} - \mathcal{M}) = 0, \hfill \\
{P_\Omega }\left( {{C_j} - {\mathcal{X}_j}{ \times _j}{\mathcal{Y}_j}} \right) + \mathcal{Q} = 0. \hfill \\ 
\end{gathered}  \right.\]
where $ \Omega ^C $ is the complement of $ \Omega $.
\par Now we establish Lemma \ref{lemma3.4} to prove that Algorithm 1 decreases the objective function value monotonically and it can converge to a KKT point of our optimization problem.
\begin{lemma}\label{lemma3.4}
	Assume that
	\[f({{\hat X}_1},{{\hat X}_2},{{\hat X}_3},{{\hat Y}_1},{{\hat Y}_2},{{\hat Y}_3},\mathcal{C}) = \sum\limits_{j = 1}^3 {\frac{{{\alpha _j}}}{{2{n_j}}}\left\| {{{\hat X}_j}{{\hat Y}_j} - {{\bar C}_j}} \right\|_F^2}  = \sum\limits_{j = 1}^3 {\sum\limits_{i = 1}^{{n_j}} {\frac{{{\alpha _j}}}{{2{n_j}}}\left\| {\hat X_j^{(i)}\hat Y_j^{(i)} - \bar C_j^{(i)}} \right\|_F^2} }. \]
is the objective function and the sequence $ \left\{ {\left( {\hat X_{^{_1}}^k,\hat X_{^{_2}}^k,\hat X_{^{_3}}^k,\hat Y_{^{_1}}^k,\hat Y_{^2}^k,\hat Y_{^{_3}}^k,{\mathcal{C}^k}} \right)} \right\} $ generated by Algorithm 1 is bounded. Then, the sequence $ \left\{ {\left( {\hat X_{^{_1}}^k,\hat X_{^{_2}}^k,\hat X_{^{_3}}^k,\hat Y_{^{_1}}^k,\hat Y_{^2}^k,\hat Y_{^{_3}}^k,{\mathcal{C}^k}} \right)} \right\} $ satisfies the following properties:
\par (1) $ f({{\hat X}_1},{{\hat X}_2},{{\hat X}_3},{{\hat Y}_1},{{\hat Y}_2},{{\hat Y}_3},\mathcal{C}) $ is monotonically decreasing. Actually, it satisfies the following inequality:
\begin{equation*}
\begin{aligned}
&\quad f(\hat X_{^{_1}}^k,\hat X_{^{_2}}^k,\hat X_{^{_3}}^k,\hat Y_{^{_1}}^k,\hat Y_{^2}^k,\hat Y_{^{_3}}^k,{\mathcal{C}^k}) - f(\hat X_{^{_1}}^{k + 1},\hat X_{^{_2}}^{k + 1},\hat X_{^{_3}}^{k + 1},\hat Y_{^{_1}}^{k + 1},\hat Y_{^2}^{k + 1},\hat Y_{^{_3}}^{k + 1},{\mathcal{C}^{k + 1}}) \hfill \\
&\geqslant \sum\limits_{j = 1}^3 {\frac{{{\alpha _j}}}{{2{n_j}}}\left\| {\hat X_{_j}^{k + 1}\hat Y_{_j}^{k + 1} - \hat X_{_j}^k\hat Y_{_j}^k} \right\|_F^2}  \geqslant 0. \hfill \\ 
\end{aligned}
\end{equation*}
\par (2) Any accumulation point $ {\left( {\hat X_{^{_1}}^*,\hat X_{^{_2}}^{\text{*}},\hat X_{^{_3}}^{\text{*}},\hat Y_{^{_1}}^{\text{*}},\hat Y_{^2}^{\text{*}},\hat Y_{^{_3}}^{\text{*}},{\mathcal{C}^*}} \right)} $ of the sequence $ \left\{ {\left( {\hat X_{^{_1}}^k,\hat X_{^{_2}}^k,\hat X_{^{_3}}^k,\hat Y_{^{_1}}^k,\hat Y_{^2}^k,\hat Y_{^{_3}}^k,{\mathcal{C}^k}} \right)} \right\} $ is a KKT point of problem \eqref{gs3.5}.
\end{lemma}
\par Therefore, the theoretical convergence of Algorithm 1 can be guaranteed. At the same time, we use the same rank estimation strategy as in \cite{ZLLZ18}




\iffalse


\subsection{Rank Estimation}\label{rtz}
In most cases, we do not know the true rank of tensor data.
Thus, it is necessary to develop a method for estimating the
rank of data. Similar to \cite{XHYS13} and \cite{WYZ12}, we adopt the rankdecreasing method to estimate the true rank of a tensor. In
this paper, to characterize the rank of data more accurately and
efficiently, we estimate the rank for each block diagonal matrix
$\bar C_j^{(i)}$. Suppose that the multi-rank of $\bar C_j^{(i)}$ is 
$$\bm{r}_j^k = \left( {\bm{r}_{1,j}^k,\bm{r}_{2,j}^k, \cdots ,\bm{r}_{{n_j},j}^k} \right),j = 1,2,3$$
at the $ k $-th iteration.We compute the eigenvalues of ${\left( {\hat X_j^{(i)}} \right)^*}\hat X_j^{(i)}$ and then sort all
these eigenvalues for each $ j $, and we can obtain
$${\lambda _{1,j}} \geqslant {\lambda _{2,j}} \geqslant  \cdots  \geqslant {\lambda _{{n_{{k_j}}},j}}, \, \, j = 1,2,3$$
where ${n_{{k_j}}} = \sum\limits_{i = 1}^{{n_j}} {r_{i,j}^k} $. Finally, we compute the quotients 
$${{\hat \lambda }_{i,j}} = {\lambda _{i,j}}/{\lambda _{i + 1,j}} \quad j = 1,2,3, \, i = 1,2,{n_{{k_j}}} - 1$$
Assume that $T _j^k = \mathop {\arg \max }\limits_{1 \leqslant i \leqslant {n_{{k_j}}} - 1} {{\hat \lambda }_{i,j}}$ and 
$$\tau _j^k = \left( {T_j^k - 1} \right){{\hat \lambda }_{T_j^k,j}}/\sum\nolimits_{i \ne T_j^k} {{{\hat \lambda }_{i,j}}} ,\quad j = 1,2,3$$
If $\tau _j^k \geqslant 10$, i.e., there being a large drop in the magnitude of the eigenvalues, we should reduce $\bm{r}_j^k$. Similar to PCA \cite{ref40}, we find ${\lambda _{{s^k},j}}$ such that it meets 
$$\sum\limits_{i = 1}^{{s^k}} {{\lambda _{i,j}}} /\sum\limits_{i = 1}^{{n_k}} {{\lambda _{i,j}}}  \geqslant 95\% $$
 Assume there are $m_{i,j}^k$ eigenvalues of ${\left( {\hat X_j^{(i)}} \right)^*}\hat X_j^{(i)}$ which belong to $\left\{ {{\lambda _{{s^k} + 1,j}}, \cdots ,{\lambda _{{n_{{k_j},j}}}}} \right\}$. Then we set $\bm{r}_{i,j}^k = \bm{r}_{i,j}^k - m_{i,j}^k$. Suppose $U_j^{(i)}\Sigma _j^{(i)}{\left( {V_j^{(i)}} \right)^T}$ is the skinny SVD of $\hat X_j^{(i)}\hat Y_j^{(i)}$. We can update
$$\hat X_j^{(i)} = U_{r_{i,j}^k,j}^{(i)}\Sigma _{r_{i,j}^k,j}^{(i)} \, , \, \hat Y_j^{(i)}{\text{ = }}\left( {V_j^{(i)}} \right)_{r_{i,j}^k,j}^T$$
where
\begin{itemize}
\item $U_{r_{i,j}^kj}^{(i)}$ consists of the first ${\bm{r}_{i,j}^k}$ columns of $U_j^{(i)}$;
\item ${\left( {V_j^{(i)}} \right)_{r_{i,j}^k,j}}$ consists of the first ${\bm{r}_{i,j}^k}$ rows of ${V_j^{(i)}}$;
\item $\Sigma _{r_{i,j}^k,j}^{(i)}$ is a diagonal matrix whose diagonal entries are the largest ${\bm{r}_{i,j}^k}$ eigenvalues of
$\Sigma _j^{(i)}$.
\end{itemize}
In this way, we can adjust the rank ${\bm{r}_{j}^k}$ and estimate the true rank of the tensor data.

\fi
























==> Chapter/section4.tex <==
\section{Numerical Experiments}

\subsection{Numerical Simulation}
Both TCTF\cite{ref} and our method TCTFG are based on the
tensor multi-rank and tubal rank definitions, depicting the
inherent low-rank structure of a tensor by characterizing the
low-rank property of their Fourier transform result. Here we
conduct experiments to compare them in detail on synthetic
data. Other methods are not compared here since they use
different tensor rank definitions. 
\par For fairness,  we randomly create a tensor $\mathcal X \in {\mathbb C^{{n_1} \times {n_2} \times {n_3}}}$\cite{KB09}:we first generate a core tensor $\mathscr E \in {\mathbb C^{{r} \times {r} \times {r}}}$ with i.i.d. Gaussian entries ($ \sim \mathcal N(0,1)$). Then, we generate matrixes ${U^{(1)}},{U^{(2)}},{U^{(3)}}$, with $U^{(i)} \in \mathbb{C}^{n_{i} \times r}$ whose entries are i.i.d. from $ \mathcal N(0,1)$ and set
$\mathcal{X}:=\mathscr{E} \times_{1} U^{(1)} \times_{2} U^{(2)} \times_{3} U^{(3)}$. We use SR to denote the sampling ratio, i.e., a percentage SR of the entries to be known and choose the support of the known entries uniformly at random among all supports of size  $S R\left(\prod_{i=1}^{3} n_{i}\right)$. We adopt the relative error
$$RSE:=\frac{\left\|\mathcal{\hat C}-\mathcal{M}\right\|_{F}}{\|\mathcal{M}\|_{F}}.$$ and as evaluation metrics. Because the Tucker rank of the third-order tensor has the following relationship with its tubal rank
\[\begin{array}{l}
r\left( {{{\mathcal M}_{(1)}}} \right) = r\left( {\bar M_3^1, \cdots ,\bar M_3^{{n_3}}} \right) \ge \max \left( {r\left( {\bar M_3^1} \right), \cdots ,r\left( {\bar M_3^{{n_3}}} \right)} \right) = rank_t^3\left( {\mathcal M} \right),\\
r\left( {{{\mathcal M}_{(2)}}} \right) = r\left( {\bar M_1^1, \cdots ,\bar M_1^{{n_1}}} \right) \ge \max \left( {r\left( {\bar M_1^1} \right), \cdots ,r\left( {\bar M_1^{{n_1}}} \right)} \right) = rank_t^1\left( {\mathcal M} \right),\\
r\left( {{{\mathcal M}_{(3)}}} \right) = r\left( {\bar M{{_2^1}^\prime }, \cdots ,\bar M{{_2^{{n_2}}}^\prime }} \right) \ge \max \left( {r\left( {\bar M_2^1} \right), \cdots ,r\left( {\bar M_2^{{n_3}}} \right)} \right) = rank_t^2\left( {\mathcal M} \right).
\end{array}\]
it is perfectly reasonable for us to generate a smaller tubal rank tensor by generating a smaller Tucker rank tensor. Finally, we uniformly select $ pn_{1}n_{2}n_{3} $ positions of $\mathcal M $ to
construct $ \Omega $, where $ p $ is the sampling ratio. 
The parameter settings used for Figure \ref{fig:1} are summarized in Table \ref{tab:1}.
\begin{table}[htbp]
	\centering
	\caption{Parameters in Numerical Simulation}
	% \begin{center}   
	\begin{tabular}{l}
		\toprule 
		\toprule
		${R^0} = 30{I_3},\, {\lambda _0} = 0.8,q = 0.8, \, {\text{Iteration = 150}},rank_{t}(\mathcal M)=(9,9,9) $                               \\
		\bottomrule 
		\bottomrule
	\end{tabular}
	% \end{center}
	\label{tab:1}
\end{table}
\par In Figure \ref{fig:1}, for our method (TCTFG), we report the recovery results of different coefficient ratios $ ({\alpha _1}:{\alpha _2}:{\alpha _3}) $ for different tensor sizes. Similarly, we also reported the recovery results of TCTF. 

\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{picture/1}
	\caption{Comparison of tensor completion on synthetic data. TCTFG recovery results for different coefficient ratios, and TCTF recovery results. Value above the bar graph: CPU time in seconds.}
	\label{fig:1}
\end{figure}


\begin{table}[htbp]
	\centering
	\caption{Numerical results for the TCTFG and TCTF.}    %表头
	\begin{center}    
		\begin{tabular}{ccccccc}
			\toprule
			\multicolumn{1}{c}{\multirow{2}{*}{$ \alpha_1:\alpha_2:\alpha_3 $}} & \multicolumn{2}{c}{${\mathcal M} \in {\mathbb {R}^{100 \times 100 \times 100}}$} 
			& \multicolumn{2}{c}{${\mathcal M} \in {\mathbb {R}^{50 \times 80 \times 100}}$} 
			& \multicolumn{2}{c}{${\mathcal M} \in {\mathbb {R}^{100 \times 80 \times 50}}$} 
			\\ \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
			% \cmidrule(r){2-3} \cmidrule(r){4-5}用来在中间间隔式插入线条 
			\multicolumn{1}{r}{}       & RSE     &time 
			                           & RSE     &time             
			                           & RSE     &time
			\\       \midrule		
	$1:1:1$ &    0.0024  &    121.61  &    0.0137  &     60.60  &    0.0111  &  61.43 \\
	
	$ 1:2:3 $ &    0.0023  &    119.24  &    0.0113  &     61.57  &    0.0148  &  61.30 \\
	
	$ 3:2:1 $ &    0.0038  &    116.94  &    0.0244  &     61.63  &    0.0157  &  62.09 \\
	
	$ 0:0:1 $ &    2.1061  &     55.47  &   19.4054  &     43.28  &    3.3068  &  25.93 \\
	
	$ 0:0:1 $(Iter: 500) &    0.7352  &    165.90  &   41.8416  &    131.99  &    3.2655  &  74.33 \\
			\bottomrule
		\end{tabular}
	\end{center}
\end{table}






\par From Figure \ref{fig:1}, we can see that TCTFG is not sensitive to the size of the coefficient ratio. Thus verifying that our method is very robust to parameters, so we will set the ratio to ${\alpha _1}:{\alpha _2}:{\alpha _3} = 1:1:1$ in future experiments. In order to compare the effect of the tensor size on the experimental results, we set three tensor sizes, which are $\mathcal {M} \in {\mathbb {R}^{100 \times 100 \times 100}},\mathcal {M} \in {\mathbb {R}^{50 \times 80 \times 100}}$, and $\mathcal {M} \in {\mathbb {R}^{100 \times 80 \times 50}}$. Graphically, although our algorithm takes a little longer to iterate 150 steps, our psnr value is much better than the TCTF algorithm. For the sake of fairness, we have deliberately set a set of $ 500 $ TCTF iterations to prevent errors caused by fewer TCTF iterations. From the results, the increase in the number of iteration steps did not reduce the psnr value obtained by the TCTF algorithm. Instead, in the tensor experiment of $\mathcal {M} \in {\mathbb {R}^{50 \times 80 \times 100}}$, the psnr value obtained by the TCTF algorithm increased as the number of iteration steps increased . In summary, our algorithm is better than the TCTF algorithm.


\begin{figure}[htbp]\label{tu2}
	\centering
	\subfloat[$ \mathcal {M} \in {\mathbb {R}^{100 \times 100 \times 100}} $]{
		\begin{minipage}[t]{0.333\linewidth}
			\centering
			\includegraphics[width=1.6in]{picture/tu2_1}
			%\caption{fig1}
		\end{minipage}%
	}%
	\subfloat[$ \mathcal {M} \in {\mathbb {R}^{50 \times 80 \times 100}} $]{
		\begin{minipage}[t]{0.333\linewidth}
			\centering
			\includegraphics[width=1.6in]{picture/tu2_2}   %指定图片大小
			%\caption{fig2}
		\end{minipage}%
	}%
	\subfloat[$\mathcal {M} \in {\mathbb {R}^{100 \times 80 \times 50}}$]{
		\begin{minipage}[t]{0.333\linewidth}
			\centering
			\includegraphics[width=1.6in]{picture/tu2_3}
			%\caption{fig2}
		\end{minipage}
	}%
	\centering
	\caption{ The RSE comparison on the synthetic data, $ p=0.6 $.}
	\label{fig:2}
\end{figure}
\begin{figure}[htbp]\label{tu2}
	\centering
	\subfloat[$ \mathcal {M} \in {\mathbb {R}^{100 \times 100 \times 100}} $]{
		\begin{minipage}[t]{0.333\linewidth}
			\centering
			\includegraphics[width=1.6in]{picture/tu3_1}
			%\caption{fig1}
		\end{minipage}%
	}%
	\subfloat[$ \mathcal {M} \in {\mathbb {R}^{50 \times 80 \times 100}} $]{
		\begin{minipage}[t]{0.333\linewidth}
			\centering
			\includegraphics[width=1.6in]{picture/tu3_2}   %指定图片大小
			%\caption{fig2}
		\end{minipage}%
	}%
	\subfloat[$\mathcal {M} \in {\mathbb {R}^{100 \times 80 \times 50}}$]{
		\begin{minipage}[t]{0.333\linewidth}
			\centering
			\includegraphics[width=1.6in]{picture/tu3_3}
			%\caption{fig2}
		\end{minipage}
	}%
	\centering
	\caption{ The RSE comparison on the synthetic data, $ p=0.8 $.}
	\label{fig:2.5}
\end{figure}

In Figure \ref{fig:2} and \ref{fig:2.5}, we report the changes in the RSE values of our algorithm and the TCTF algorithm with the number of iteration steps. It can be seen from the figure that no matter the size of the tensor, our algorithm is iterating around $ 40 $ steps. The RES value tends to $ 0 $, but the RSE value of the TCTF algorithm is at least 2; and when the tensor is $\mathcal {M} \in {\mathbb {R}^{50 \times 80 \times 100}}$, its RSE The value reaches 4 or more, indicating that it also has certain requirements on the tensor size. In summary, our algorithm is better than the TCTF algorithm. We can know from Figure \ref{fig:2} and Figure \ref{fig:2.5} that the more data is missing, the worse the effect of the TCTF algorithm, which further verifies that the TCTF algorithm does not use the tensor data more comprehensively.


 \subsection{Image Simulation}
In this part, Assume that $ \mathcal{\hat C} $ is the recovered tensor of$ \mathcal M $. We employ the peak signal-to-noise ratio (PSNR), defined as
$$\operatorname{PSNR}=10 \log _{10}\left(\frac{n_{1} n_{2} n_{3}\|\mathcal{M}\|_{\infty}^{2}}{\|\hat{\mathcal{C}}-\mathcal{M}\|_{F}^{2}}\right)$$
and the algorithm running time , the value of PSNR and the value of RSE to evaluate these methods. we randomly sample all testing
images by the sampling ratio $ p = 0.7 $.


\begin{figure}[htbp]
	\centering
	\subfloat{
		\begin{minipage}[t]{0.5\linewidth}
			\centering
			\includegraphics[width=2.3in]{picture/picture_bar3}
			%\caption{fig1}
		\end{minipage}%
	}%
	\subfloat{
		\begin{minipage}[t]{0.5\linewidth}
			\centering
			\includegraphics[width=2.3in]{picture/picture_bar3_rse}   %指定图片大小
			%\caption{fig2}
		\end{minipage}%
	}%
	\centering
	\caption{ Comparison between algorithms for the different Image}
	\label{fig:5}
\end{figure}
\input{Chapter/tu}
\begin{table}[htbp]
	\centering
	\caption{Numerical results for the different Image.}    %表头
	\begin{center}    
		\begin{tabular}{cccccccccc}
			\toprule
			\multicolumn{1}{c}{\multirow{2}{*}{Image}} & \multicolumn{3}{c}{TCTFG} & \multicolumn{3}{c}{TCTF} & \multicolumn{3}{c}{Tmac} 
			\\ \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
			% \cmidrule(r){2-3} \cmidrule(r){4-5}用来在中间间隔式插入线条 
			\multicolumn{1}{r}{} & PSNR      & RSE     &time 
			&PSNR         & RSE         &time             
			&PSNR         & RSE         &time
			\\       \midrule	
			Flower & {\bf 32.12 } & {\bf 0.08 } &     13.63  &     30.96  &      0.09  &     14.03  &     30.27  &      0.10  &     14.30  \\
			
			Desert & {\bf 34.66 } & {\bf 0.04 } &     12.21  &     30.73  &      0.06  &     12.66  &     28.30  &      0.08  &     12.60  \\
			
			River otter & {\bf 32.55 } & {\bf 0.07 } &     13.05  &     29.07  &      0.10  &     12.71  &     28.93  &      0.10  &     13.56  \\
			
			Viaduct & {\bf 36.17 } & {\bf 0.04 } &     12.71  &     32.59  &      0.05  &     12.48  &     32.91  &      0.05  &     13.02  \\
			
			House & {\bf 32.69 } & {\bf 0.04 } &     11.85  &     28.84  &      0.07  &     12.58  &     28.75  &      0.07  &     13.19  \\
			
			Man & {\bf 29.34 } & {\bf 0.06 } &     12.09  &     26.15  &      0.09  &     13.49  &     27.34  &      0.08  &     14.23  \\
			
        	human & {\bf 29.64 } & {\bf 0.07 } &     17.19  &     27.92  &      0.08  &     14.29  &     28.56  &      0.07  &     13.91  \\

            girl & {\bf 30.66 } & {\bf 0.06 } &     12.79  &     26.41  &      0.10  &     12.80  &     28.00  &      0.09  &     13.10  \\
			\bottomrule
		\end{tabular}
	\end{center}
\end{table}







\par We show the repair results of the eight test images in Figure \ref{fig:3}. Our method is better than TCTF and TMac. TMac expands the tensor data directly into matrixs and apply matrix nuclear norm  to preserve the
low-rank structure of the tensor, which may destroy multi-data structures and cause performance degradation \cite{ZEAHK14,KBHH13}. Based on the recent results of tensor decomposition, TCTF and our method avoid the loss of tensor structure information \cite{ZEAHK14,KBHH13}, so as to obtain better repair results. However, TMac is superior to TCTF in the recovery of human images. Because TCTF only considers the rank related to module 3, but ignores the rank related to module 1 and module 2, the information is not enough. Our method takes into account all the ranks of module 1 to module 3, and more comprehensively reflects the information of tensors. Therefore, our method is superior in the restoration of both characters and landscape images.


\subsection{\textcolor{red}{Video Simulation}}
The data between two adjacent frames of the video usually does not change much. To study the stability of the video data, we calculate the data pairs of the corresponding positions between two adjacent frames. The difference for two adjacent frames of the video slots($ k $ and $ k+1 $) is equal to
\begin{equation*}
day(i,j,k)=| {\mathcal C}_3^k(i,j)-{\mathcal C}_3^{k+1}(i,j) |.
\end{equation*}
The smaller the $ day(i, j, k) $, the more stable the data between two adjacent frames of the video at frame $ k $. By computing the normalized difference values between two adjacent frames, we measure the stability between two adjacent frames of the video at frame $ k $ as
\begin{align*}
\Delta gap(i, j, k)=\frac{|{\mathcal C}_3^k(i,j)-{\mathcal C}_3^{k+1}(i,j)|}{\max\limits _{1 \leqslant i \leqslant n_1,1 \leqslant j \leqslant n_2, 1 \leqslant k \leqslant n_3-1}|{\mathcal C}_3^k(i,j)-{\mathcal C}_3^{k+1}(i,j)|}.
\end{align*}
where $ \max\limits _{1 \leqslant i \leqslant n_1,1 \leqslant j \leqslant n_2, 1 \leqslant k \leqslant n_3-1}|{\mathcal C}_3^k(i,j)-{\mathcal C}_3^{k+1}(i,j)| $ is the maximal gap between any two adjacent frames of the video in the video data. We plot the CDF of $ \Delta day(i, j, k) $ in Figure \ref{fig:tu4_1}. The X-axis represents the normalized difference values between two adjacent frames slots, i.e., $ \Delta day(i, j, k) $. The Y-axis represents the cumulative probability. we can see that the value $ \Delta day(i, j, k)<0.5 $ is is nearly about 80\%. These results indicate that the temporal stability exists in the real video data. So here we add ST-TCTFG for comparison. Because the video data has only temporal characteristics, here we let $ T_{1} = T_{2} = 0 $.
\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{picture/tu4_1}
	\caption{Empirical study with real video data}
	\label{fig:tu4_1}
\end{figure}



\input{Chapter/tu2}

\begin{table}[htbp]
	\centering
	\caption{Numerical results of four algorithms on video recovery.}    %表头
	\begin{center}    
		\begin{tabular}{cccccccccc}
			\toprule
			\multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{3}{c}{Hall} & \multicolumn{3}{c}{Highway} & \multicolumn{3}{c}{Waterfall} 
			\\ \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
			% \cmidrule(r){2-3} \cmidrule(r){4-5}用来在中间间隔式插入线条 
			\multicolumn{1}{r}{} & PSNR      & RSE     &time 
			&PSNR         & RSE         &time             
			&PSNR         & RSE         &time
			\\       \midrule		
	TCTFG & {\bf 30.294 } & {\bf 0.016 } &    18.491  & {\bf 35.641 } & {\bf 0.007 } &    17.997  & {\bf 30.355 } & {\bf 0.023 } &    48.786  \\

ST-TCTFG & {\bf 31.113 } & {\bf 0.015 } &    19.717  & {\bf 39.534 } & {\bf 0.005 } &    21.056  & {\bf 34.551 } & {\bf 0.014 } &    56.250  \\

TCTF &    24.987  &     0.030  &    24.899  &    28.498  &     0.017  &    25.732  &    23.190  &     0.053  &    95.235  \\

TMac &    24.899  &     0.031  &    20.532  &    38.040  &     0.006  &    22.160  &    25.680  &     0.040  &    73.453  \\
			\bottomrule
		\end{tabular}
	\end{center}
\end{table}



\par As shown in figure \ref{fig:5}, we set p=0.5, 0.7, and 0.9, respectively, to display frame 18 of the test video. From the recovery results, our method performs better in filling the missing values of the three test sequences. It handles frame details well. On the PSNR and RSE measure, our method is also optimal, consistent with the observations in figure \ref{fig:5}. Especially when p=0.9, our method has more advantages. The results of video repair are also consistent with the results of image repair, indicating that our method can perform the tensor better and run more efficiently. In our improved algorithm, we use the spatio-temporal features of video data, so the recovery effect is better.

\subsection{\textcolor{red}{Internet Traffic Simulation}}
	we model the traffic data as a 3-way tensor $ \mathcal{M} \in {\mathbb R^{o \times t \times d}} $. 

\begin{minipage}[b]{0.3\linewidth}
	\includegraphics[width=0.8\linewidth]{picture/tensor}
	%\caption{Traffic tensor model.}
\end{minipage}
\hfill
\begin{minipage}[b]{0.65\linewidth}
	Here `$ o $' corresponds to $ N \times N $ OD pairs, and there are `$ d $' days to consider with each day having `$ t $' time intervals. We randomly selected three weeks of data in the public traffic trace data Abilene\cite{TAODC}. For the Abilene trace, $ t = 288,o = 121,d = 7 $. 
\end{minipage}

Similar to spatiotemporal analysis of video data, We also plot the CDF of $ \Delta gap(i, j, k) $ in Figure \ref{fig:8}. 
\begin{figure}[htbp]
	\centering
	\begin{minipage}[b]{1\linewidth}
		\subfloat[the first week]{
			\begin{minipage}[b]{0.33\linewidth}
				\centering
				\includegraphics[width=\linewidth]{picture/dataX2}
		\end{minipage}}
		\subfloat[the second week]{    	
			\begin{minipage}[b]{0.33\linewidth}
				\centering
				\includegraphics[width=\linewidth]{picture/dataX3}
		\end{minipage}}
			\subfloat[The third week]{ 
			\begin{minipage}[b]{0.33\linewidth}
				\centering
				\includegraphics[width=\linewidth]{picture/dataX4}
		\end{minipage}}
	\end{minipage}
	\vfill
	\caption{An empirical study of three sets of real traffic data.}
	\label{fig:8}
\end{figure}
  we can see that the value $ \Delta gap(i, j, k)<0.5 $ is is nearly about 60\%. These results indicate that the temporal stability exists in the real traffic data. So here we add TCTFG$ - $improve for comparison.

\begin{figure}[htbp]
	\centering
	\begin{minipage}[b]{1\linewidth}
		\subfloat[RSE]{
			\begin{minipage}[b]{0.49\linewidth}
				\centering
				\includegraphics[width=\linewidth]{picture/tuX2_1}
		\end{minipage}}
		\subfloat[Computation time]{    	
			\begin{minipage}[b]{0.49\linewidth}
				\centering
				\includegraphics[width=\linewidth]{picture/tuX2_2}
		\end{minipage}}
	\end{minipage}
	\vfill
	\caption{One sequence step with different sampling ratio for the first week of data.}
	\label{fig:9}
\end{figure}

\begin{figure}[htbp]
	\centering
	\begin{minipage}[b]{1\linewidth}
		\subfloat[RSE]{
			\begin{minipage}[b]{0.49\linewidth}
				\centering
				\includegraphics[width=\linewidth]{picture/tuX3_1}
		\end{minipage}}
		\subfloat[Computation time]{    	
			\begin{minipage}[b]{0.49\linewidth}
				\centering
				\includegraphics[width=\linewidth]{picture/tuX3_2}
		\end{minipage}}
	\end{minipage}
	\vfill
	\caption{One sequence step with different sampling ratio for the second week of data.}
	\label{fig:10}
\end{figure}

\begin{figure}[htbp]
	\centering
	\begin{minipage}[b]{1\linewidth}
		\subfloat[RSE]{
			\begin{minipage}[b]{0.49\linewidth}
				\centering
				\includegraphics[width=\linewidth]{picture/tuX4_1}
		\end{minipage}}
		\subfloat[Computation time]{    	
			\begin{minipage}[b]{0.49\linewidth}
				\centering
				\includegraphics[width=\linewidth]{picture/tuX4_2}
		\end{minipage}}
	\end{minipage}
	\vfill
	\caption{One sequence step with different sampling ratio for the third week of data.}
	\label{fig:11}
\end{figure}

From Figure \ref{fig:9} to Figure \ref{fig:11} we can see that our algorithm has a good ability to capture global information in traffic data to recover lost data with high accuracy. As can be seen from Figure \ref{fig:9}(a) to Figure \ref{fig:11}(a), among all the implemented tensor completion algorithms, our algorithm is basically the best. And in the case of high sample rate, our algorithm reflects its superiority.
















==> Chapter/section5.tex <==
\section{Conclusion}
In this paper, we propose a generalized tubal rank based on the tensor tubal rank. The tubal rank only considers the frontal slice of the tensor, and we consider the horizontal, lateral and frontal slices of the tensor 
to use the tensor data more comprehensively. Compared with Tucker rank of tensor, our method avoids destroying the low rank structure inherent in tensor. In addition, we have also improved the algorithm for data with certain spatiotemporal characteristics. Experimental results show that the performance of our proposed method is significantly better than existing methods in the open literature.
